CUDA: Curriculum of Data Augmentation for Long-Tailed Recognition

Class imbalance problems frequently occur in real-world tasks, and conventional deep learning algorithms are well known for performance degradation on imbalanced training datasets. To mitigate this problem, many approaches have aimed to balance among given classes by re-weighting or re-sampling training samples. These re-balancing methods increase the impact of minority classes and reduce the influence of majority classes on the output of models. However, the extracted representations may be of poor quality owing to the limited number of minority samples. To handle this restriction, several methods have been developed that increase the representations of minority samples by leveraging the features of the majority samples. Despite extensive recent studies, no deep analysis has been conducted on determination of classes to be augmented and strength of augmentation has been conducted. In this study, we first investigate the correlation between the degree of augmentation and class-wise performance, and find that the proper degree of augmentation must be allocated for each class to mitigate class imbalance problems. Motivated by this finding, we propose a simple and efficient novel curriculum, which is designed to find the appropriate per-class strength of data augmentation, called CUDA: CUrriculum of Data Augmentation for long-tailed recognition. CUDA can simply be integrated into existing long-tailed recognition methods. We present the results of experiments showing that CUDA effectively achieves better generalization performance compared to the state-of-the-art method on various imbalanced datasets such as CIFAR-100-LT, ImageNet-LT, and iNaturalist 2018.

==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/command/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.


% Customized Math
\DeclareMathOperator{\Tr}{Tr}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\let\ab\allowbreak

\newcommand{\trace}{\Tr}


==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/command/mycommand.tex <==
\usepackage{microtype}
\usepackage{geometry}
% \usepackage{subfig}
\usepackage{booktabs} 
\usepackage{bbm}
\usepackage{mathtools}
% \usepackage{amsthm}
\usepackage{nccmath}
\usepackage{setspace}

\usepackage{caption}
\usepackage{subcaption}

\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}
\newcommand{\algcapsty}[1]{\small\sffamily\bfseries{#1}}
\SetAlCapSty{algcapsty}

\usepackage[T1]{fontenc}
\usepackage{wrapfig,lipsum,booktabs}

% \usepackage{natbib}
\usepackage{soul}
\usepackage{dsfont}
\usepackage{enumerate}
\usepackage{enumitem}

% \usepackage{kotex}
% \usepackage{hyperref}
% \usepackage[hidelinks]{hyperref}
\usepackage{amsmath}
% \usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{arabtex}
\usepackage{bbm}
\usepackage{dsfont}
\usepackage[Symbol]{upgreek}
\usepackage{lscape}
\usepackage{caption}
\usepackage{balance}
\usepackage{xspace}
\usepackage{float}



\usepackage{wasysym}
\usepackage[table,xcdraw,dvipsnames]{xcolor}
\usepackage{multirow}
\usepackage{array, boldline, rotating}

\usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand{\ds}[1]{\mathds{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\bb}[1]{\mathbbm{#1}}

% %%%%%% Theorem Related Things %%%%%%
% \theoremstyle{plain}
% \newtheorem{thm}{Theorem}
% \newtheorem{cor}{Corollary}
% \newtheorem{lem}{Lemma}
% \newtheorem{prop}{Proposition}

% \theoremstyle{definition}
% \newtheorem{defn}{Definition}
% \newtheorem{assum}{Assumption}



% Citation

% \let\oldeqcite\cite
% \renewcommand*\cite[1]{(\oldcite{#1})}
\let\oldeqref\eqref
\renewcommand*\eqref[1]{(\ref{#1})}

% % Highlight (incl. note)
\newcommand{\smnote}[1]{\textbf{\textcolor{Cyan}{SM: #1}}}
\newcommand{\jwnote}[1]{\textbf{\textcolor{Orange}{JW: #1}}}
\newcommand{\eg}{\emph{e.g.,~}}
\newcommand{\ie}{\emph{i.e.,~}}


% % Separation (paragraph)
\newcommand{\myparagraph}[1]{\vspace{0.07cm}\noindent\textbf{#1}~}

% % math op.

% % Font
\def\code#1{\texttt{#1}}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}

% % % Definition
% \theoremstyle{definition}




\newcommand{\thickhline}{\hlineB{4}}
\newcommand{\bfcode}[1]{\code{\textbf{#1}}}


\definecolor{LightCyan}{rgb}{0.88,1,1}

==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/main/00_abstract.tex <==
Class imbalance problems frequently occur in real-world tasks, and conventional deep learning algorithms are well known for performance degradation on imbalanced training datasets. 
To mitigate this problem, many approaches have aimed to balance among given classes by \emph{re-weighting} or \emph{re-sampling} training samples. 
These re-balancing methods increase the impact of minority classes and reduce the influence of majority classes on the output of models. 
However, the extracted representations may be of poor quality owing to the limited number of minority samples.
To handle this restriction, several methods have been developed that increase the representations of minority samples by leveraging the features of the majority samples.  
Despite extensive recent studies, no deep analysis has been conducted on determination of classes to be augmented and strength of augmentation has been conducted.
In this study, we first investigate the correlation between the degree of augmentation and class-wise performance, and find that the proper degree of augmentation must be allocated for each class to mitigate class imbalance problems. Motivated by this finding, we propose a simple and efficient novel curriculum, which is designed to find the appropriate per-class strength of data augmentation, called \alg: \textbf{\code{CU}}rriculum of \textbf{\code{D}}ata \textbf{\code{A}}ugmentation for long-tailed recognition.
\alg can simply be integrated into existing long-tailed recognition methods. We present the results of experiments showing that \alg~effectively achieves better generalization performance compared to the state-of-the-art method on various imbalanced datasets such as CIFAR-100-LT, ImageNet-LT, and iNaturalist 2018.  
\footnote{Code is available at \href{https://github.com/sumyeongahn/CUDA_LTR}{Link}}
\vspace{-10pt}


==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/main/01_intro.tex <==
\section{Introduction}
\label{sec:intro}

Deep neural networks (DNNs) have significantly improved over the past few decades on a wide range of tasks~\cite{he2017mask, redmon2017yolo9000, qi2017pointnet}. This effective performance is made possible by come from well-organized datasets such as MNIST~\cite{lecun1998gradient}, CIFAR-10/100~\cite{krizhevsky2009learning}, and ImageNet~\cite{russakovsky2015imagenet}. However, as \citet{van2018inaturalist} indicated, gathering such balanced datasets is notoriously difficult in real-world applications. In addition, the models perform poorly when trained on an improperly organized dataset, \eg in cases with class imbalance, because minority samples can be ignored due to their small portion.

The simplest solution to the class imbalance problem is to prevent the model from ignoring minority classes. To improve generalization performance, many studies have aimed to emphasize minority classes or reduce the influence of the majority samples. Reweighting~\cite{cao2019learning, menon2021longtail} or resampling~\cite{buda2018systematic, van2007experimental} are two representative methods that have been frequently applied to achieve this goal. (i) \emph{Reweighting} techniques increase the weight of the training loss of the samples in the minority classes. (ii) \emph{Resampling} techniques reconstruct a class-balanced training dataset by upsampling minority classes or downsampling majority classes. 

Although these elaborate rebalancing approaches have been adopted in some applications, limited information on minority classes due to fewer samples remains problematic. To address this issue, some works have attempted to spawn minority samples by leveraging the information of the minority samples themselves. For example,~\citet{chawla2002smote, ando2017deep} proposed a method to generate interpolated minority samples. Recently~\cite{kim2020m2m, chu2020feature, park2022majority} suggested enriching the information of minority classes by transferring information gathered from majority classes to the minority ones. For example, \citet{kim2020m2m} generated a balanced training dataset by creating adversarial examples from the majority class to consider them as minority.

Although many approaches have been proposed to utilize data augmentation methods to generate various information about minority samples, relatively few works have considered the influence of the degree of augmentation of different classes on class imbalance problems. In particular, few detailed observations have been conducted as to which classes should be augmented and how intensively.

\begin{figure*}[t]
    \centering
    \vspace{-10pt}
    % \includegraphics[width=.9\textwidth]{fig/intuition.pdf}
    \includegraphics[width=.9\textwidth]{fig/intuition_revise.pdf}
    \vspace{-5pt}
    \caption{Motivation of \alg.
    If one half of the classes (\eg class indices in $0$-$49$) are strongly augmented, the \rebut{averaged accuracy} of the other half of the classes (\ie in $50$-$99$) increases. \rebut{The heatmaps in the first and the second rows present the accuracy for class indices in $0$-$49$ and $50$-$99$, respectively. Also, each point in the plots means the accuracy under corresponding augmentation strength.} This phenomenon is also observed in the imbalanced case in which the top first half (major\rebut{; the first row}) have more samples than the second half classes (minor\rebut{; the second row}). Setup and further analysis are described in~\autoref{app:figure_1}.}
    \vspace{-20pt}
    \label{fig:intuition}
\end{figure*}

To this end, we first consider that controlling the strength of class-wise augmentation can provide another dimension to mitigate the class imbalance problem. In this paper, we use the number of augmentation operations and their magnitude to control the extent of the augmentation, which we refer to herein as its strength, \eg a strength parameter of $2$ means that two randomly sampled operations with a pre-defined magnitude index of $2$ are used.

Our key finding is that class-wise augmentation improves performance in the non-augmented classes while that for the augmented classes may not be significantly improved, and in some cases, performances may even decrease. As described in~\autoref{fig:intuition}, regardless of whether a given dataset is class imbalanced, conventional class imbalance methods show similar trends: when only the major classes are strongly augmented (\eg  strength $4$), the performance of majority classes decreases, whereas that for the minority classes have better results. \rebut{To explain this finding, we further} find that \rebut{strongly augmented classes get diversified feature representation,} preventing the growth of the norm of a linear classifier for corresponding classes. \rebut{As a result, the softmax outputs of the strongly augmented classes are reduced, and thus the accuracy of those classes decreases.}
% diversifying \rebut{images (that incur diversified representation vectors)} of augmented classes prohibit the growth of the norm of a linear classifier for corresponding classes, and this classifier tends to increase the logit value for the non-augmented classes. 
It is described in~\autoref{app:figure_1}. 
This result motivates us to find the proper augmentation strength for each class to improve the performance for other classes while maintaining its own performance.

\myparagraph{Contribution.}
We propose a simple algorithm called \textbf{\code{CU}}rriculum of \textbf{\code{D}}ata \textbf{\code{A}}ugmentation (\alg) to find the proper class-wise augmentation strength for long-tailed recognition. Based on our motivation, we have to increase the augmentation strength of majorities for the performance of minorities when the model successfully predicts the majorities. On the other hand, we have to lower the strength of majorities when the model makes wrong predictions about majorities. 
The proposed method consists of two modules, which compute a level-of-learning score for each class and leverage the score to determine the augmentation. 
Therefore, \alg increases and decreases the augmentation strength of the class that was successfully and wrongly predicted by the trained model. 
To the best of our knowledge, this work is the first to suggest a class-wise augmentation method to find a proper augmentation strength for class imbalance problem.

We empirically examine performance of \alg on synthetically imbalanced datasets such as CIFAR-100-LT~\cite{cao2019learning}, ImageNet-LT~\cite{liu2019large}, and a real-world benchmark, iNaturalist 2018~\cite{van2018inaturalist}. With the high compatibility of \alg, we apply our framework to various long-tailed recognition methods and achieve better performance compared to the existing long-tailed recognition methods. Furthermore, we conduct an extensive exploratory analysis to obtain a better understanding of \alg. The results of these analyses verify that \alg exhibits two effects that mitigate class imbalance, including its balanced classifier and improved feature extractor.


==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/main/02_related.tex <==
\vspace{-10pt}
\section{Related works}
\label{sec:related}
\vspace{-10pt}

\myparagraph{Long-tailed Recognition (LTR).} % TODO: JONGWOO
The datasets with class imbalances can lead DNNs to learn biases toward training data, and their performance may decrease significantly on the balanced test data. To improve the robustness of such models to imbalance, LTR methods have been evolving in two main directions: (1) reweighting~\citep{cui2019class, cao2019learning, park2021influence} methods that reweight the loss for each class by a factor inversely proportional to the number of data points, and (2) resampling methods~\citep{kubat1997addressing, chawla2002smote, ando2017deep} that balance the number of training samples for each class in the training set. However, studies along these lines commonly sacrifice performance on majority classes to enhance that on minority classes, because the overfitting problem occurs with limited information on minority classes as a result of increasing the weight of a small number of minority samples.

Several methods have recently been developed to alleviate the overfitting issues in various categories: (1) two-stage training~\cite{cao2019learning, kang2019decoupling, liu2019large}, (2) ensemble methods~\cite{zhou2020bbn, xiang2020learning, wang2021longtailed, cai2021ace}, and (3) contrastive learning approach~\cite{kang2021exploring, cui2021parametric, zhu2022balanced, li2022nested, li2022targeted}. To re-balance the classifier layers after achieving a good representation on the imbalanced training dataset in an early phase, \citet{cao2019learning} proposed deferred resampling (DRS) and reweighting (DRW) approaches. \citet{kang2019decoupling} decoupled the learning procedure into representation learning and training linear classifier, achieved higher performance than previous balancing methods. \citet{wang2021longtailed} and \citet{cai2021ace} suggested efficient ensemble methods using multiple experts with a routing module and a shared architecture for experts to capture various representations. \citet{liu2022selfsupervised} found that self-supervised representations are more robust to class imbalance than supervised representations, and some works have developed supervised contrastive learning methods~\citep{khosla2020supervised} for imbalanced datasets~\citep{cui2021parametric, zhu2022balanced, li2022targeted}.

Another line of research has considered augmentation methods in terms of both input and feature spaces \cite{kim2020m2m, chu2020feature, li2021metasaug}. Recently, \citet{park2022majority} mixed minority and majority images by using CutMix with different sampling strategies to enhance balancing and robustness simultaneously. These methods commonly focus on utilizing the rich context of majority samples to improve the diversity of minority samples. Moreover, these augmentation-based methods are relatively in easy to apply orthogonally with other LTR methods.
% Our work is also along on this direction which is easy to apply orthogonally with other long-tailed methods.

\myparagraph{Data Augmentation (DA).} % TODO : SM #최대한 짧게 적음
DA has been studied to mitigate overfitting which may occur due to a lack of data samples. 
% Especially, DA is widely studied in vision tasks such as image classification. 
Some works have been proposed to erase random parts of images to enhance the generalization performance of neural networks~\cite{devries2017improved, zhong2020random, kumar2017hide, choe2019attention}. Recently, variants of MixUp~\citep{zhang2017mixup} have been proposed; this method combines two images with specific weights~\citep{tokozume2018between, guo2019mixup, takahashi2018ricap, devries2017improved, verma2019manifold}. By aggregating two approaches, CutMix~\citep{yun2019cutmix} was proposed to erase and replace a small rectangular part of an image into another image.
In another line of research, methods have been proposed to automatically configure augmentation operations~\cite{cubuk2019autoaugment, lim2019fast, li2020dada, hataya2020faster, gudovskiy2021autodo}. In addition, \citet{cubuk2020randaugment} randomly selected augmentation operations using the given hyperparameters of the number of sampling augmentation and their magnitudes. Recently, class-wise or per-sample auto-augmentation methods have also been proposed~\cite{cheung2021adaaug, rommel2021cadda}.

==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/main/03_method.tex <==
\section{\textbf{\underline{CU}}rriculum of \textbf{\underline{D}}ata \textbf{\underline{A}}ugmentation for Long-Tailed Recognition}
\label{sec:method}
\vspace{-10pt}


% Algorithm design overview
The core philosophy of \alg is to \emph{``generate an augmented sample that becomes the most difficult sample without losing its original information.''} In this section, we describe design of \alg in terms of two parts: (1) a method to generate the augmented samples based on the given strength parameter, and (2) a method to measure a Level-of-Learning (LoL) score for each class.


\subsection{Problem Formulation of Long-tailed Recognition}
% \subsection{Preliminary}
% First of all, we describe basic notations which will be used in this section. 

% \myparagraph{Long-tailed Recognition (LTR).}
Suppose that the training dataset $\mc{D} = \{(x_i,y_i)\}_{i=1}^N$ is composed of images with size $d$, $x_i\in \bb{R}^{d}$, and their corresponding labels $y_i\in \{1,...,C\}$. $\mc{D}_c \subset \mc{D}$ is a set of class $c$, \ie $\mc{D}_{c} = \{(x,y) | y = c, (x,y) \in \mc{D}\}$. Without loss of generality, we assume $|\mc{D}_1| \ge |\mc{D}_2|  \ge \cdots \ge |\mc{D}_C|$, where $|\mc{D}|$ denotes the cardinality of the set $\mc{D}$. We denote the $N_{\text{max}} \coloneqq |\mc{D}_1|$ and $N_{\text{min}} \coloneqq |\mc{D}_C|$. LTR algorithms, $\mc{A}_{\text{LTR}}(f_{\theta},\mc{D})$, mainly focus on training the model $f_{\theta}$ with parameter $\theta$ when the class distribution of training dataset $\mc{P}_{\text{train}}(y)$ and test dataset $\mc{P}_{\text{test}}(y)$ are not identical. More precisely, $\mc{P}_{\text{train}}(y)$ is highly imbalanced while $\mc{P}_{\text{test}}(y)$ is balanced, \ie uniform distribution.
% The main objective of LTR is to train the model to be performs well under the uniform class distribution $\mc{P}_{\text{test}}(y)$. 

\subsection{Curriculum of Data Augmentation}

In this section, we describe our proposed DA with strength parameter, and the methods used to measured the LoL score. Then, we integrate the two methods in a single framework to propose \alg.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{fig/algorithm.pdf}
    \caption{Algorithm overview. \alg is composed of two main parts: (1) strength-based augmentation and (2) Level-of-Learning (LoL) score. To control the difficulty of augmented images, strength-based augmentation utilizes two values, the number of augmentations and their magnitudes. We use the strength-based augmentation module to score the LoL. Based on the measured LoL score, \alg generates adequately augmented images for LTR algorithms.}
    \label{fig:algorithm}
    \vspace{-10pt}
\end{figure*}


\myparagraph{DA with a strength parameter.}
Let us assume that there exist pre-defined $K$ augmentation operations. We utilize visual augmentation operations which is indexed as $k \in \{1, \cdots, K\}$, \eg Gaussian blur, Rotation, Horizontal flip. Each augmentation operation $\mc{O}_{k}^{m_k(s)} : \bb{R}^{d} \to \bb{R}^{d}$ has its own pre-defined augmentation magnitude function $m_k(s)$ where the strength parameter $s \in \{0,...,S\}$. These operations are described in detail along with each magnitude functions in~\autoref{app:augmentation}.

Given an augmentation strength parameter $s$ and an input image $x$, we model a sequence of augmentation operations $\mc{O}(x;s)$  as follows:
\begin{equation*}
    \mc{O}(x;s) = \mc{O}^{m_{k_s}(s)}_{k_s} \circ \mc{O}^{m_{k_{s-1}}(s)}_{k_{s-1}} \circ \cdots \circ \mc{O}^{m_{k_{1}}(s)}_{k_1}(x), \quad  k_i \sim \text{Cat}(K,\mc{U}(K)) \quad \forall i = \{ 1,\ldots, s\}, % \mc{U}(K)
\end{equation*}

where, $\text{Cat}(\cdot)$ and $\mc{U}(\cdot)$ denote categorical and discrete uniform distributions, respectively. 
% Note that we sample the augmentation operations $(k_1, \ldots , k_s)$ from uniform distribution $1/\binom{K}{s}$, which is denoted by $\text{Choice}(K,s)$.
% uniform categorical distribution $\text{Cat}(\cdot, \cdot)$ without replacement.
The sequential augmentation operation $\mc{O}(x;s)$ samples $s$ operations from the categorical distribution when the probability of seeing the operations follows uniform distribution. 
% Sequential operation is depicted in the left side of ~\autoref{fig:algorithm}.
As depicted on the left side~\autoref{fig:algorithm}, suppose that the random sampled augmentations $k_1$, $k_2$, and $k_3$ are brightness, X-shift, and Y-shift, respectively. Then, $\mc{O}(x;3)$ outputs an image in which bright is raised by $m_{\text{bright}}(3)$ and moved by $m_{\text{x-shift}}(3)$ on the x-axis and shifted by $m_{\text{y-shift}}(3)$ on the y-axis.


\scalebox{0.8}{
\begin{minipage}{0.75\textwidth}
\begin{algorithm}[H]
    \DontPrintSemicolon
    \SetAlgoLined
    \SetNoFillComment
    \LinesNotNumbered 
    \caption{\textbf{CU}rriculum of \textbf{D}ata \textbf{A}ugmentation}
    \label{alg:cuda}
    \KwInput{LTR algorithm $\mc{A}_{\text{LTR}}(f,\mc{D})$, training dataset $\mc{D}=\{(x_i,y_i)\}_{i=1}^N$, train epochs $E$, aug. probability $p_{\text{aug}}$, threshold $\gamma$, number of sample coefficient $T$. }
    \KwOutput{trained model $f_\theta$}
    % \KwOutput{$\bar{\mc{D}}$}
    \textbf{Initialize:} $L_c^0 = 0$ $\forall c \in \{1,...,C\}$\\
    \For{$e \le E$} 
    {   
        Update $L_c^e = V_{\text{LoL}}(\mc{D}_{c}, L_c^{e-1}, f_{\theta}, \gamma, T)$ \quad $\forall c $\tcp*{Alg.~\ref{alg:LoL}} 
        Generate  $\mc{D}_{\text{CUDA}} = \{(\bar{x}_i, y_i)| (x_i,y_i) \in \mc{D} \}$ where   
        \begin{equation*}
            \bar{x}_i = 
            \begin{cases} 
                \mc{O}(x_i,L_{y_{i}}^{e}) &\text{with prob. } p_{\text{aug}} \\
                x_{i}   &\text{otherwise.}
            \end{cases}
        \end{equation*} \\
        Run LTR algorithm using $\mc{D}_{\text{CUDA}}$, \ie $\mc{A}_{\text{LTR}}\left(f_\theta,\mc{D}_{\text{CUDA}} \right)$.
    }
\end{algorithm}
\end{minipage}}
\hfill
\scalebox{0.75}{
\begin{minipage}{0.52\textwidth}
\begin{algorithm}[H]
    \setstretch{1.177}
    \DontPrintSemicolon
    \SetAlgoLined
    \SetNoFillComment
    \LinesNotNumbered 
    \caption{$V_{\text{LoL}}$: Update LoL score}
    \label{alg:LoL}
    \KwInput{$\mc{D}_{c}$, $L$, $f_{\theta}$, $\gamma$, $T$}
    \KwOutput{updated $L$}
    \textbf{Initialize:} check $= 1$ \\
    \For{$l \le L$}   
    {   
        \textcolor{blue}{/* $V_{\text{correct}}(\mc{D}_{c},l,f_\theta,T)$  */} \\
        Sample $\mc{D}_{c}' \subset \mc{D}_c$  s.t. $|\mc{D}_{c}'| = T(l+1) $ \\
        Compute $v = \sum_{x \in \mc{D}_{c}'} \mathbbm{1}_{\{f(\mc{O}(x;l) = c\}}$ \\
        \If{ $v \le \gamma T (l+1)$}
        % \If{\sum_{x \in \mc{D}_{c}'} \mathbbm{1}_{\{f(\mc{O}(x;l) = c\}} > \gamma T(l+1)}
        {check $\leftarrow 0$; \textbf{break}}
        % \If{$V_{Correct}(\mc{D}_c,l,f_\theta, T) \ge \gamma T(l+1)$}
        % {pass}
        % \Else
        % {
        %     $L \leftarrow L -1$
        % }
    }
    \textbf{if} check $= 1$ \textbf{then} $L \leftarrow L+1$ \\
    \textbf{else} $L \leftarrow L-1$
\end{algorithm}
\end{minipage}}

\myparagraph{Level-of-Learning (LoL).} To control the strength of augmentation properly, we check whether the model can correctly predict augmented versions without losing the original information. To enable this, we define the LoL for each class $c$ at epoch $e$, \ie $L_c^e$, which is adaptively updated as the training continues as follows:
% To control the strength of augmentation properly, we have to check whether the model can correctly predict augment version while do not lose the information of original image. To enable this, we define the Level of Learning (LoL) for each sample $(x_i,y_i)$ at epoch $e$, \ie $L_i^e$, which is adaptively updated as the training goes on, as follows:
\begin{equation*}
    L_{c}^{e} =  V_{\text{LoL}}(\mc{D}_c, L_c^{e-1}, f_{\theta}, \gamma, T),
\end{equation*}





where 
\begin{equation*}
    \centering
    \resizebox{0.98\linewidth}{!}{
    $V_{\text{LoL}}(\mc{D}_c,L_c^{e-1},f_{\theta}, \gamma, T) = 
    \begin{cases}
        L_c^{e-1} + 1 \quad \text{if } V_{\text{Correct}}(\mc{D}_{c}, l ,f_{\theta}, T) \geq \gamma T (l + 1) \quad \forall l \in \{0,...,L_{c}^{e-1}\} \\
        L_c^{e-1} - 1 \quad \text{otherwise}
    \end{cases}$.}
\end{equation*}

Here, $\gamma \in [0, 1]$ is threshold hyperparameter, $T$ is coefficient of the number of samples used to updating LoL. $V_{\text{correct}}$ is a function which outputs the number of correctly predicted examples by the model $f_{\theta}$ among $l+1$ randomly augmented samples with strength $l$. $V_{\text{correct}}$ is defined as: 
\begin{equation*}
    V_{\text{Correct}}(\mc{D}_{c}, l, f_{\theta}, T) = \textstyle \sum_{x \in \mc{D}_{c}'} \mathbbm{1}_{\{ f_{\theta}(\mc{O}(x;l)) = c\}} \quad \text{where } \mc{D}_{c}' \subset \mc{D}_c.
\end{equation*}
Note that $\mc{D}_{c}'$ is a randomly sampled subset of $\mc{D}_{c}$ with replacement and its size is $T(l+1)$.
% Note that $V_{\text{Correct}}(\mc{D}_{c}, l, f_{\theta},T)$ is the number of correctly predicted examples by the model $f_{\theta}$ among the $l+1$ random augment examples with strength $l$ %, $\{\bar{x}_j = \mc{O}(x;l)| x \in \mc{D}_{c}\}_{j=1}^{l+1}$, as below:
% as below:
% \begin{equation*}
%     V_{\text{Correct}}(\mc{D}_{c}, l, f_{\theta}, T) = \textstyle \sum_{j=1}^{T(l+1)} \mathbbm{1}_{\{ f_{\theta}(\mc{O}(x_{j};l)) = c\}}  \quad x_{j} \in \mc{D}_{c},
% \end{equation*}
% where we conduct computation of $V_{\text{correct}}$ with randomly selected data through sampling with replacement from $\mc{D}_{c}$. 




The key philosophy of this criterion is two fold. (1) If samples in the class $c$ are trained sufficiently with an augmentation strength of $L_{c}^{e}$, the model is ready to learn a more difficult version with augmentation strength of $L_{c}^{e+1} \leftarrow L_{c}^{e}+1$. In contrast, if the model predicts incorrectly, it should re-learn the easier sample with an augmentation strength of $L_{c}^{e+1} \leftarrow L_{c}^{e}-1$. (2) As the strength parameter increases, the number of candidates for the sequential augmentation operation $\mc{O}(x; L)$ increases exponentially. For example, the amount of increment is $N^{L} (N - 1)$ when $L$ is increases to $L+1$. To control the LoL in a large sequential augmentation operation space, we take more random samples to check as the strength parameter gets bigger. In our experiments, linearly increasing the number of samples to evaluate corresponding to the strength with a small additional computation time was sufficient. $V_{\text{LoL}}$ is described in  \autoref{fig:algorithm} and Algorithm~\ref{alg:LoL}.

% where $x_j \in \mc{D}_{c}$ is randomly sampled data with replacement from $\mc{D}_{c}$. 

% where the $V_{\text{Correct}}(x_i, y_i, s, f_{\theta})$ is the number of correctly predicted examples by the model $f_{\theta}$ among the $s+1$ random samples of $\mc{O}(x_i;s)$. The key philosophy of this criterion is two-fold. (1) If a sample is trained sufficiently with augmentation strength $L$, \ie if the trained model correctly predict until $L$, it means that the model is ready to learn a more difficult version with augmentation strength $L+1$. On the other hand, if the model predicts wrongly, the model should re-learn the much easier samples. (2) As the augmentation strength grows, the number of candidates for augmented samples exponentially increases. For instance, the amount of increment is $P(K, L+1) - P(K, L)$ when $L$ increases to $L+1$, where $P(K, L) := \frac{K!}{(K-L)!}$ represents permutation.  To check the LoL with enormous sample space, we increase the number of random samples to check as the augmentation strength become larger.

\myparagraph{Curriculum of DA.} By combining two components, including DA with a strength parameter and LoL, our \alg provides class-wise adaptive augmentation to enhance the performance of the others without losing its own information. As shown in~\autoref{fig:algorithm} and Algorithm~\ref{alg:cuda}, we measure the LoL score $L_c$ for all classes in the training dataset to determine the augmentation strength for every epoch. Based on $L_c$, we generate the augmented version $\mc{O}(x; L_c)$ for $x \in \mc{D}_{c}$ and train the model with the augmented samples. Additionally, we randomly use the original sample instead of the augmented sample with probability $p_{\text{aug}}$ so that the trained models do not forget the original information. In our experiments, this operation improved performance robustly on a wide range of $p_{\text{aug}}$ values. The results are provided in Section~\ref{exp:analysis}.

\myparagraph{Advantage of \alg design.}
Our proposed approach mainly has three advantages. (1) \alg adaptively finds proper augmentation strengths for each class without need for a validation set. 
(2) Following the spirits of existing curriculum learning methods~\cite{hacohen2019power, zhou2020curriculum, wu2021when}, \alg enables modeling by first presenting easier examples earlier during training to improve generalization. This encourages the model to learn difficult samples (\ie within high augmentation strength) better. (3) Moreover, owing to the universality of data augmentation, \alg is easily compatible with other LTR algorithms, such as~\cite{cao2019learning, ren2020balanced, wang2021longtailed}.

% pseudocode - appendix에...
% DoL 기반 학습 mechanism
% 그림으로 설명



% Algorithm design philosophy overview
% The core philosophy of \alg~ is \emph{``Constructing curriculum which making easy samples (major class) be difficult, and difficult samples (minor class) not be difficult.''} This is based on the intuition that samples that have already been well-learned are difficult to have a significant impact on the model. In other words, easy samples have to be more difficult samples to give the model positive influence, and in contrast, difficult samples can have a big impact on themselves. In this section, we describe our intuition in detail and the proposed algorithm, curriculum data augmentation for long-tailed learning in details. 

% \subsection{Notations}
% \smnote{augmentation 관련 notation}
% \jwnote{$N_{max}, N_{min}$ 등의 표현도 정리해주면 좋을듯}
% % Before diving into the method, we briefly summarize the basic notations and problem settings. Suppose that the training dataset $\mc{D} = \{(x_i,y_i)\}_{i=1}^N$ composed of image $x_i\in \bb{R}^{W \times H \times C}$ and its corresponding label $y_i\in \{1,...,C\}$ is given. When $\mc{D}_c$ means a set of class $c$, \ie $\mc{D}_{c} = \{(x_i,y_i) | y_i = c\}$, we mainly focus on the case $|\mc{D}_{M}| \gg |\mc{D}_{m}|$ case, where $M$ and $m$ is the major and minor set, respectively. Without loss of generality, we denote $c=1$ to $C$ by sorted meaning, \ie $c=1$ is the most common and $c=C$ is the most rare class. 

% \begin{figure*}[t]
%     \centering
%     \subfloat[A]{\includegraphics[width=0.245\textwidth]{fig/n_sample_Loss.pdf}
%     \label{fig:per_class_loss}}
%     \subfloat[B]{\includegraphics[width=0.245\textwidth]{fig/n_sample_L2.pdf}
%     \label{fig:per_class_grad_norm}}
%     \subfloat[C]{\includegraphics[width=0.245\textwidth]{example-image-a}
%     \label{fig:c}}
%     \subfloat[D]{\includegraphics[width=0.245\textwidth]{example-image-b}
%     \label{fig:d}}
%     \caption{Caption}
%     \label{fig:method}
% \end{figure*}
% \subsection{Make easy samples be more difficult, difficult samples not be more difficult} 
% Here, we design our algorithm by answering the following questions: (1) Do easy samples give less influence to the model? (2) Can making easy samples be difficult improve feature extractor? And, consequently it can mitigate class imbalance problem? and (3) How can we make the per-sample curriculum based on the degree of difficulty? Experimental results in this section come from CIFAR-100-LT benchmark with ResNet32 backbone networks. Detail experimental settings, such as learning rate, are described in Section~\ref{sec:exp}.

% \myparagraph{Do easy samples have less effect on the model?} 
% To check the impact of easy samples and difficult samples, we examine two types of metrics, gradient-norm and loss. For simplicity, we report the average scores for each class. As in Figure~\ref{fig:per_class_loss}, we can find that major classes have lower losses than the minor classes. Furthermore, as in Figure~\ref{fig:per_class_grad_norm}, small loss from the major  classes does not significantly change the model, which causes a negative effect on limiting the feature extractor. Therefore, by modifying easy samples to difficult ones, we can make the feature extractor change more.


% \myparagraph{Can we improve the feature extractor by making easy samples be difficult?} 
% The second question is divisible into two sub-questions. First, is it possible to obtain better feature extractor by making easy samples be difficult?  Second, the strengthened feature extractor can mitigate the class imbalance problem? To answer those two questions, we examine four types of feature extractor which is trained by using, w/o augmented, uniformly augmented, strong augmentation for major class, and strong augmentation for minor class. As in Figure~\smnote{Figure} ---
% \smnote{Freezing 실험으로 FE 가중요한 부분이다.}



% \myparagraph{Designing per-sample curriculum based on the degree of difficulty.} 
% \smnote{difficult sample을 만드는 주안점은 2가지. (1) 충분히 어려워야 한다. (2) 어렵지만, 너무 어려워지면 안된다. }


% \subsection{Curriculum Data Augmentation for Long-tailed Recognition}
% \smnote{알고리즘 설명 (1) rand augment parameter, strength score, cutmix 어떤식으로 쓸 수 있는지 등}


==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/main/04_exp.tex <==
\section{Experiments}
\label{sec:exp}
In this section, we present empirical evaluation, the results of which demonstrate the superior performance of our proposed algorithm for class imbalance. We first describe the long-tailed classification benchmarks and implementations in detail (Section~\ref{exp:set}). Then, we describe the experimental results on several synthetic (CIFAR-100-LT, ImageNet-LT) and real-world (iNaturalist 2018) long-tailed benchmark datasets in Section~\ref{exp:result}. Moreover, we conduct additional experiments to obtain a better understanding of \alg, and this analysis is provided in Section~\ref{exp:analysis}.

\input{tab/cifar_200ep}

\subsection{Experimental setup}\label{exp:set}
\vspace{-10pt}
\myparagraph{Datasets.}
We evaluate \alg on the most commonly used long-tailed image classification tasks: CIFAR-100-LT~\cite{cao2019learning}, ImageNet-LT~\cite{liu2019large}, and iNaturalist 2018~\cite{van2018inaturalist}. CIFAR-100-LT and ImageNet-LT are provided with imbalanced classes by synthetically sampling the training samples. CIFAR-100-LT is examined with various imbalance ratios $\{100, 50, 10 \}$, where an imbalance ratio is defined as $N_{\text{max}} / N_{\text{min}}$. iNaturalist 2018 is a large-scale real-world dataset includes natural long-tailed imbalance. We utilize the officially provided datasets.

\myparagraph{Baselines.} We compare \alg with previous long-tailed learning algorithms , including cross-entropy loss (CE), two-stage approaches: CE-DRW~\cite{cao2019learning} and cRT~\cite{kang2019decoupling}, balanced loss approaches: LDAM-DRW~\cite{cao2019learning} and Balanced Softmax (BS; \citealt{ren2020balanced}), the ensemble method: RIDE with three experts~\cite{wang2021longtailed}, resampling algorithms: Remix~\cite{chou2020remix} and CMO~\cite{park2022majority}, and contrastive learning-based approach: BCL~\cite{zhu2022balanced}. We integrate \alg with CE, CE-DRW, LDAM-DRW, BS, RIDE, and BCL algorithms. For longer epochs, we compare \alg with PaCo~\cite{cui2021parametric}, BCL, and NCL~\cite{li2022nested}, by combining \alg with BCL and NCL. For a fair comparison of the computational cost, we train the network with the official one-stage implementation of RIDE (\ie without distillation and routing).

\myparagraph{Implementation.} For CIFAR-100-LT dataset, almost all implementations follow the general setting from~\citet{cao2019learning}, whereas cRT~\cite{kang2019decoupling}, BCL, NCL and RIDE follow the settings used in their original implementation. Following \citet{cao2019learning}, we use ResNet-32~\cite{he2016deep} as a backbone network for CIFAR-100-LT. The network is trained on SGD with a momentum of $0.9$ and a weight decay of $2\times10^{-4}$. The initial learning rate is $0.1$ and a linear learning rate warm-up is used in the first $5$ epochs to reach the initial learning rate. During training over $200$ epochs, the learning rate is decayed at the $160$th and $180$th epochs by $0.01$. 
For the ImageNet-LT and iNaturalist, the ResNet-50 is used as a backbone network and is trained for $100$ epochs. The learning rate is decayed at the $60$th and $80$th epochs by $0.1$. As with CIFAR, for cRT, RIDE, and BCL, we follow the original experimental settings of the official released code. For the hyperparameter values of \alg, we apply a $p_{\text{aug}}$ of $0.5$ and $T$ of $10$ for all experiments. For $\gamma$, we set the values as $0.6$ for CIFAR-100-LT and $0.4$ for ImageNet-LT and iNaturalist 2018. The detailed implementation for baselines are in \autoref{app:implementation}.

\subsection{Experimental Results}
\label{exp:result}
In this section, we report the performances of the methods compared on the CIFAR-100-LT, ImageNet-LT, and iNaturalist 2018. We include four different categories of accuracy: all, many, med(ium), and few. Each represents the average accuracy of all samples, classes containing more than $100$ samples, $20$ to $100$ samples, and under $20$ samples, respectively.

\input{tab/real_world}
\input{tab/aug_result_other_config}

\myparagraph{CIFAR-100-LT.} In \autoref{tab:cifar_200ep}, we report the performance when \alg~is applied to the various algorithms: CE, CE-DRW~\cite{cao2019learning}, LDAM-DRW~\cite{cao2019learning}, BS~\cite{ren2020balanced}, RIDE~\cite{wang2021longtailed} with 3 experts, RIDE+CMO~\cite{park2022majority}, and BCL~\cite{zhu2022balanced}.
Compared to the cases without \alg, balanced validation performance is increased when we apply the proposed approach. 

Recently, some works \cite{cui2021parametric, alshammari2022long, zhu2022balanced, li2022nested} have shown impressive performances with diverse augmentation strategies and longer training epochs. For a fair comparison with these methods, we examine \alg using the same experimental setups from PaCo (\citealt{cui2021parametric}; 400 epochs with batch size of 64). Table~\ref{tab:cifar_other} shows that augmented images using \alg can enhance LTR performance compared to the other baselines. In particular, \alg with NCL obtains the best performance over $400$ epochs. As noted by~\citet{li2022nested}, the NCL algorithm utilizes six times as much memory compared to the vanilla architecture with three experts. Hereinafter in large-scale benchmarks, we focus on the cases with similar network size. 

\myparagraph{ImageNet-LT and iNaturalist 2018.} To evaluate the performance of \alg on larger datasets, we conduct experiments on ImageNet-LT~\cite{liu2019large} and iNaturalist 2018~\cite{van2018inaturalist}. Table~\ref{tab:in_inat} summarizes the performance of various LTR methods and the performance gain when integrated with \alg. Our proposed method consistently improves performance regardless of the LTR method and target dataset by simply adding class-wise data augmentation without complicated methodological modification. Additionally, to evaluate the performance gain of \alg on other architectures, we experiment with \alg on ImageNet-LT with ResNet-10~\cite{liu2019large} and ResNeXt-50~\cite{xie2017aggregated}, as reported in \autoref{app:analysis}.

\input{tab/norm_softmax}
\input{tab/curriculum}

\vspace{-2pt}
\subsection{Analysis}\label{exp:analysis}
\vspace{-2pt}
We design our analyses to answer the following questions. (1) How does \alg perform? (2) Does \alg perform better than other augmentation methods? (3) How does LoL score change over training epochs when combined with various LTR methods? (4) Which part of \alg is important to improved performance? These analyses provide additional explanations to understand \alg. All experiments are conducted on CIFAR-100-LT with imbalance ratio of $100$.

\myparagraph{How does \alg mitigate the class imbalance problem?}
To deeply understand \alg, we observe two types of metrics: 
% (1) variance of classifier weight L1-norm, 
(1) variance of weight L1-Norm of linear classifier between each class
% (2) feature alignment gain (\ie cosine similarity with and without \alg) on validation dataset. 
(2) feature alignment gain for each class (\ie cosine similarity with and without \alg) on validation dataset.
The classifier weight norm is usually used to measure how balanced the model consider the input from a class-wise perspective~\cite{kang2019decoupling, alshammari2022long}. Feature alignment, especially feature cosine similarity amongst samples belonging to the same class, is a measure of the extent to which the extracted features are aligned~\cite{oh2021boil}. As shown in~\autoref{fig:output_analysis}, \alg has two forces for alleviating imbalance. For all cases, \alg reduces the variance of the weight norm (\ie balance the weight norm), and thus the trained model consider the minority classes in a balanced manner. Note that because LDAM-DRW and RIDE utilize a cosine classifier (\ie utilizing L2 normalized linear weight), their standard deviation scale is quite different from those other methods. Because LDAM-DRW, BS, and RIDE include balancing logic in their loss function, they exhibit lower variance reduction compared to the CE and CE-DRW. Second, as shown in the bottom row in~\autoref{fig:output_analysis}, \alg obtains feature alignment gains for almost all classes. This shows that \alg facilitates a network to learn to extract meaningful features.

\myparagraph{Compared with other augmentations.} To verify the impact of \alg, we examine the other augmentation methods as follows. We compare five augmentation methods, including AutoAugment (AA, \citealt{cubuk2019autoaugment}), Fast AutoAugment (FAA, \citealt{lim2019fast}), DADA~\cite{li2020dada}, RandAugment (RA, \citealt{cubuk2020randaugment}), and the proposed method \alg. Because AA, FAA, and DADA provide their policies searched by using CIFAR, SVHN (for AA), and ImageNet, we leverage their results. Furthermore, RA suggests using their parameter $(n,m)=(1,2)$ for CIFAR, and we follow their guidelines. As shown in~\autoref{tab:dataug}, even though the \rebut{automated augmentation methods} use additional computation resources to search, \alg outperforms the other pre-searched augmentations. This shows that \alg is computationally efficient.

% Furthermore, we check whether \alg is compatibly applicable with AA. This analysis is conducted on the CIFAR-100-LT with imbalance ratio $100$. As described in \autoref{tab:dataug}, 

\myparagraph{Dynamics of LoL score.}
We evaluate how LoL scores vary with algorithms: CE, CE-DRW, LDAM-DRW, BS, and RIDE. Note that we set a lower class index (\ie $0$) as the most common class (\ie the number of samples is $500$), while an index of $100$ represents the rarest class (\ie with five samples). As described in~\autoref{fig:curriculum}, as training progressed, the LoL score of all algorithms increase. After learning rate decay (\ie 160 epoch) all algorithms are able to learn to classify minority classes more easily than before. In particular, except for BS, the majority classes of most algorithms show a steep increment. The reason that BS exhibit a similar increasing speed for majority and minority classes is that it includes a module to balance the impact of majority and minority samples. \rebut{Furthermore, we found that CE-DRW and BS have similar end average accuracy in the case of applying \alg but different LoL score dynamics. We can conclude that LoL score on one category of classes has a high correlation with the performance of opposite classes from the observation that CE-DRW has higher and lower performance gain for many and few, respectively, than BS.} 
% Moreover, because RIDE can promote when all experts satisfying promotion criterion, its increasing speed is moderate.

\begin{figure}[!t]
    \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=1.\linewidth]{fig/aug_prob.pdf}
            \vspace{-15pt}
            \caption{Aug prob. $p_{\text{aug}}$.}
            \label{fig:aug_prob}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=1.\linewidth]{fig/num_test.pdf}
            \vspace{-15pt}
            \caption{Num test $T$.}
            \label{fig:num_test}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
          \includegraphics[width=1.\linewidth]{fig/acc_rate.pdf}
          \vspace{-15pt}
            \caption{Accept rate $\gamma$.}
          \label{fig:acc_rate}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
          \includegraphics[width=1.\linewidth]{fig/hyperopt_revise.pdf}
          \vspace{-15pt}
            \caption{Curriculum.}
          \label{fig:hyper_opt}
    \end{subfigure}
    \vspace{-5pt}
    \caption{Additional analysis of \alg. (a) sensitivity of augmentation probability $p_{\text{aug}}$, (b) sensitivity analysis of number of sample coefficient $T$, (c) sensitivity of acceptance threshold $\gamma$, and (d) impact of curriculum. The dotted lines in (a), (b) and (c) represents the performance of CE.}
    \label{fig:analysis}
    \vspace{-13.5pt}
\end{figure}

\myparagraph{Parameter sensitivity.} For further analysis, we conduct a sensitivity analysis of hyperparameters in \alg. More precisely, we study three kinds of parameters, including augmentation probability $p_{\text{aug}}$~(\autoref{fig:aug_prob}), number of tests $T$~(\autoref{fig:num_test}), and LoL update threshold $\gamma$~(\autoref{fig:acc_rate}). We examine each hyperparameter sensitivity on a \alg case with RIDE and the remainder of the hyperparameters are fixed to the default values in Section~\ref{exp:set}. All results show that the performance gains of \alg decreases if the parameters are adjusted to make the augmentation too strong or weak. For example, the augmentation strength of all classes steeply increases when $\gamma$ becomes small. The strength cannot increase when $\gamma$ becomes large, and thus it cannot improve the performance of the model. Moreover, as shown in~\autoref{fig:num_test}, the performance of \alg increases as $T$ increases. However, larger $T$ spends computational overhead, we set $T$ as $10$ and obtained cost-effective performance gain.

\myparagraph{Impact of curriculum.} In addition to studying the impact of \alg, we examine its performance component-wise. In particular, we test the case where class-wise augmentation strength is searched based on the hyperparameter optimization algorithm. We check five cases overall: \rebut{baseline} algorithm, hyperparameter optimization (HO), re-searched DADA for CIFAR-100-LT, \alg without curriculum, (\ie re-training utilizing the final augmentation strength of \alg), and \alg. \rebut{We provide detailed description for each method in \autoref{app:hyperopt}.} As described in~\autoref{fig:hyper_opt}, \alg finds better augmentation strengths compare to the hyperparameter search case. This means that \alg exhibits not only a lower searching time but also obtains better augmentation strength. Moreover, by comparing the performance of with or without curriculum, the curriculum also can provide additional advance to the model to achieve better generalization. Additionally, as \autoref{fig:curriculum}, lower augmentation strength at the beginning of training is more effective than static higher augmentation strength. These results are consistent with the results of previous studies on curriculum learning methods~\cite{ zhou2020curriculum}.

==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/main/05_conclusion.tex <==
% \vspace{-12.5pt}
\section{Conclusion}
\label{sec:conclusion}
% \vspace{-12.5pt}
In this study, we proposed \alg to address the class imbalance problem. The proposed approach is also compatible with existing methods. To design a proper augmentation for LTR, we first studied the impact of augmentation strength for LTR. We found that the strength of augmentation for a specific type of class (\eg major class) could affect the performance of the other type (\eg minor class). From this finding, we designed \alg to adaptively find an appropriate augmentation strength without any further searching phase by measuring the LoL score for each epoch and determining the augmentation accordingly. To verify the superior performance of proposed approach, we examined each performance with various methods and obtained the best performance among the methods compared, including synthetically generated and real-world benchmarks. Furthermore, from our analyses, we validated that our \alg enhanced balance and feature extraction ability, which can consistently improve performance for majority and minority classes.

\section*{Acknowledgement}
This work was supported by Institute of Information \& communications Technology Planning \& Evaluation (IITP) grant funded by the Korea government (MSIT) (No.2019-0-00075, Artificial Intelligence Graduate School Program (KAIST), 10\%) and the Institute of Information \& communications Technology Planning \& Evaluation (IITP) grant funded by the Korea government (MSIT) (No. 2022-0-00871, Development of AI Autonomy and Knowledge Enhancement for AI Agent Collaboration, 90\%)

==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/tab/aug_description.tex <==
\begin{figure}[!t]
  \centering
  \begin{subfigure}[b]{0.16\linewidth}
      \includegraphics[width=\linewidth]{fig/aug_ex/raw.png}
      \caption{Raw}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/Flip.png}
          \caption{Flip}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/Mirror.png}
          \caption{Mirror}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/EdgeEnhance.png}
          \caption{Edge Enhance}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/Detail.png}
          \caption{Detail}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/Smooth.png}
          \caption{Smooth}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/AutoContrast.png}
          \caption{AutoContrast}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/Equalize.png}
          \caption{Equalize}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/Invert.png}
          \caption{Invert}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/GaussianBlur.png}
          \caption{Gaussian Blur}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/ResizeCrop.png}
          \caption{Resize Crop}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/Rotate.png}
          \caption{Rotate}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/Posterize.png}
          \caption{Posterize}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/Solarize.png}
          \caption{Solarize}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/SolarizeAdd.png}
          \caption{SolarizeAdd}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/Color.png}
          \caption{Color}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/Contrast.png}
          \caption{Contrast}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/Brightness.png}
          \caption{Brightness}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/Sharpness.png}
          \caption{Sharpness}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/ShearX.png}
          \caption{ShearX}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/ShearY.png}
          \caption{ShearY}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/TranslateXabs.png}
          \caption{Translate X}
  \end{subfigure}
  \begin{subfigure}[b]{0.16\linewidth}
          \includegraphics[width=\linewidth]{fig/aug_ex/TranslateYabs.png}
          \caption{Translate Y}
  \end{subfigure}
\end{figure}


\begin{table}[t!]
\caption{Description of augmentation operations utilized in \alg. We show the examples of each augmentation with maximum augmentation parameters.}
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{c|c|c}
\thickhline
% \multicolumn{1}{c||}{\code{Raw img}} & \multicolumn{2}{c}{\parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/raw.png}}} \\ \hline
Operation &  Parameter &  Description \\ \hline
\code{Flip} 
& On/Off
& Flip top and bottom \\ \hline
% &\parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/Flip.png}} &

\code{Mirror} 
& On/Off
& Flip left and right \\ \hline
% & \parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/Mirror.png}}\\ \hline

\code{Edge Enhancement} 
& On/Off
& Increasing the contrast of the pixels around the targeted edges \\ \hline
% & \parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/EdgeEnhance.png}}&

\code{Detail} 
& On/Off   
& Utilize convolutional kernel $[[0, -1, 0], [-1, 10, -1], [0, -1, 0]]$ \\ \hline
% &\parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/Detail.png}}\\ \hline

\code{Smooth} 
& On/Off   
& Utilize convolutional kernel $[[1, 1, 1], [1, 5, 1], [1, 1, 1]]$\\ \hline
% &\parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/Smooth.png}}&

\code{AutoContrast} 
& On/Off
& Remove a specific percent of the lightest and darkest pixels\\ \hline
% & \parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/AutoContrast.png}}\\ \hline

\code{Equalize} 
& On/Off   
& apply non-linear mapping to make uniform distribution\\ \hline
% & \parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/Equalize.png}}&

\code{Invert} 
& On/Off   
& Negate the image\\ \hline
% &\parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/Invert.png}}\\ \hline

\code{Gaussian Blur} 
& [0,2]
& Blurring an image using Gaussian function\\ \hline
% & \parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/GaussianBlur.png}}&

\code{Resize Crop} 
& [1,1.3]  
& Resizing and center random cropping\\ \hline
% & \parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/ResizeCrop.png}}\\ \hline

\code{Rotate} 
& [0,30]
& Rotate the image\\ \hline
% &\parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/Rotate.png}}&

\code{Posterize} 
& [0,4]
& Reduce the number of bits for each channel\\ \hline
% & \parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/Posterize.png}}\\ \hline

\code{Solarize} 
& [0,256]
& Invert all pixel values above a threshold\\ \hline
% & \parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/Solarize.png}}&

\code{SolarizeAdd} 
& [0,110]
& Adding value and run solarize\\ \hline
% & \parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/SolarizeAdd.png}}\\ \hline

\code{Color} 
& [0.1, 1.9]
& Colorize gray scale values\\ \hline
% &\parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/Color.png}}&

\code{Contrast} 
& [0.1,1.9]
& Distance between the colors\\ \hline
% & \parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/Contrast.png}}\\ \hline

\code{Brightness} 
& [0.1,1.9]
& Adjust image brightness\\ \hline
% & \parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/Brightness.png}}&

\code{Sharpness} 
& [0.1,1.9]
& Adjust image sharp\\ \hline
% & \parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/Sharpness.png}}\\ \hline

\code{Shear X} 
& [0,0.3]
& Shearing X-axis\\ \hline
% &\parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/ShearX.png}}&

\code{Shear Y} 
& [0,0.3]
& Shearing Y-axis\\ \hline
% &\parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/ShearY.png}}\\ \hline

\code{Translate X} 
& [0,100]
& Shift X-axis\\ \hline
% & \parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/TranslateXabs.png}}&

\code{Translate Y} 
& [0,100]
& Shifting Y-axis\\ \hline
% & \parbox[c]{6em}{\includegraphics[width=0.15\textwidth]{fig/aug_ex/TranslateYabs.png}}\\ \hline

\thickhline
\end{tabular}
}\label{tab:aug_description}
% \end{subfigure}
\end{table}


==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/tab/aug_result_other_config.tex <==
\begin{center}
\begin{table}[t!]
\begin{minipage}{0.252\linewidth}
\caption{Comparison for CIFAR-LT-100 performance on ResNet-32 with 400 epochs. }
\label{tab:cifar_other}
\centering
\resizebox{1.0\columnwidth}{!}{
% \begin{tabular}{lccc}g
% \thickhline

% \multirow{2}{*}{Algorithm}  &  \multicolumn{3}{c}{CIFAR-100} \\ \cline{2-4} 
% \begin{tabular}{l||ccc|ccc}
\begin{tabular}{l||cc}
% \begin{tabular}{p{0.3\textwidth}||>
% {\centering}p{0.08\textwidth}>
% {\centering\arraybackslash}p{0.08\textwidth}}
\thickhline
\multirow{2}{*}{Algorithm} 
& \multicolumn{2}{c}{Imbalance Ratio} \\
\cline{2-3} 

                            & 100 & 50 \\ \hline
% BS~\cite{park2022majority}$^\dagger$
%                             & $50.0$     & $53.0$    & $60.2$ & -     & -    & - \\
PaCo
                            & $52.0$     & $56.0$      \\
BCL
                            & $52.6$ & $57.2$  \\
% LTR-WB\cite{alshammari2022long}$^\star$
%                             & $53.4$     & $57.7$    & $68.7$  \\
% NCL (single)~\cite{li2022nested}$^\dagger$
%                             & $53.3$     & $56.8$    & - \\
NCL
                            & $\underline{54.2}$ & $\underline{58.2}$   \\ \hline
% \rowcolor[HTML]{EFEFEF} 
\rowcolor{LightCyan} 
BCL + CUDA     
                            & $53.5$     & $57.4$   \\
% \rowcolor[HTML]{EFEFEF}
\rowcolor{LightCyan} 
NCL + CUDA     
                            & $\mathbf{54.8}$     & $\mathbf{59.6}$   \\ \thickhline

\end{tabular}
}
\end{minipage}
\hspace{0.15in}
\begin{minipage}{0.695\linewidth}
\caption{Augmentation analysis on CIFAR-100-LT with IR 100. AA~\cite{cubuk2019autoaugment}, FAA~\cite{lim2019fast}, DADA~\cite{li2020dada}, and RA~\cite{cubuk2020randaugment} with $n=1, m=2$ policies are used. C, S, I represent CIFAR, SVHN, and ImageNet policy.}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{lccccccccccccc>{\columncolor{LightCyan}}c}
% \begin{tabular}{p{0.2\textwidth}>
% {\centering}p{0.15\textwidth}>
% {\centering}p{0.15\textwidth}>
% {\centering}p{0.15\textwidth}>
% {\centering\arraybackslash}p{0.15\textwidth}}
\thickhline
% \multirow{2}{*}{Algorithm}
& \multirow{2}{*}{Vanilla} &&  \multicolumn{3}{c}{AA} &&  \multicolumn{2}{c}{FAA} &&  \multicolumn{2}{c}{DADA} &&  \multirow{2}{*}{RA}  &  \\ 
% \cmidrule{4-6}  \cmidrule{8-9}  \cmidrule{11-12} 
                            
                            & && C & S & I && C & I && C & I &&&\multirow{-2}{*}{\cellcolor{LightCyan}CUDA} \\ \hline
CE                          
                            & $38.7$ && $41.7$    & $40.7$    & $40.1$    && $\underline{42.3}$ & $40.8$    && $41.0$    & $41.2$    && $40.5$ & $\mathbf{42.7}$ \\
CE-DRW                          
                            & $41.4$ && $\underline{46.5}$    & $44.7$    & $45.5$    && $46.3$ & $44.8$    && $45.6$    & $45.7$    && $45.8$ & $\mathbf{47.4}$ \\
LDAM-DRW                          
                            & $42.5$ && $\underline{47.0}$    & $44.7$    & $44.9$    && $46.6$ & $45.6$    && $45.9$    & $46.5$    && $44.0$ & $\mathbf{47.2}$ \\
BS                          
                            & $43.3$ && $\underline{47.0}$    & $46.1$    & $45.5$    && $46.5$ & $45.0$    && $45.0$    & $46.9$    && $45.2$ & $\mathbf{47.7}$ \\
RIDE (3 experts)                           
                            & $49.7$ && $49.5$    & $47.3$    & $45.5$    && $49.8$ & $\underline{50.6}$    && $50.4$    & $50.5$    && $47.9$ & $\mathbf{50.7}$ \\

% rand aug 2-14 / 36.5 / 43.3  /40.8  /43.7 / 42.0
\thickhline
\end{tabular}
\label{tab:dataug}}
\end{minipage}
\end{table}
\vspace{-30pt}
\end{center}







% \begin{table}[t!]
% % \begin{minipage}[b]{1.0\linewidth}
% \caption{Comparison between other augmentation methods. We utilize augmentation policies proposed in each paper, which is obtained by using the full balanced dataset.}
% \centering
% \resizebox{0.7\columnwidth}{!}{
% \begin{tabular}{lcccccccccccccc}
% % \begin{tabular}{p{0.2\textwidth}>
% % {\centering}p{0.15\textwidth}>
% % {\centering}p{0.15\textwidth}>
% % {\centering}p{0.15\textwidth}>
% % {\centering\arraybackslash}p{0.15\textwidth}}
% \thickhline
% % \multirow{2}{*}{Algorithm}
% & \multirow{2}{*}{Vanilla} &&  \multicolumn{3}{c}{AA} &&  \multicolumn{2}{c}{FAA} &&  \multicolumn{2}{c}{DADA} &&  \multirow{2}{*}{RA}  & \multirow{2}{*}{CUDA} \\
% \cmidrule{4-6}  \cmidrule{8-9}  \cmidrule{11-12}
                            
%                             & && C & S & I && C & I && C & I  \\ \hline
% CE                          
%                             & $38.7$ && $41.7$    & $40.7$    & $40.1$    && $\mathbf{42.3}$ & $40.8$    && $41.0$    & $41.2$    && $36.5$ & $\underline{42.0}$ \\
% CE-DRW                          
%                             & $41.4$ && $\underline{46.5}$    & $44.7$    & $45.5$    && $46.3$ & $44.8$    && $45.6$    & $45.7$    && $43.3$ & $\mathbf{47.4}$ \\
% LDAM-DRW                          
%                             & $42.5$ && $\underline{47.0}$    & $44.7$    & $44.9$    && $46.6$ & $45.6$    && $45.9$    & $46.5$    && $40.8$ & $\mathbf{47.2}$ \\
% BS                          
%                             & $41.6$ && $\underline{47.0}$    & $46.1$    & $45.5$    && $46.5$ & $45.0$    && $45.0$    & $46.9$    && $43.7$ & $\mathbf{47.7}$ \\
% RIDE (3 experts)                           
%                             & $49.7$ && $49.5$    & $47.3$    & $45.5$    && $49.8$ & $\underline{50.6}$    && $50.4$    & $50.5$    && $42.0$ & $\mathbf{50.7}$ \\
% % BCL
% %                             & $48.6$    & $48.7$    & $48.6$    & $49.4$ & $48.1$    & $48.6$    & $49.1$    & $48.8$ & $52.3$ \\

% \thickhline
% \end{tabular}
% }\label{tab:dataug}
% % \end{minipage}
% \end{table}


% \begin{table}[t!]
% \begin{minipage}[b]{1.0\linewidth}
% \caption{Validation accuracy on CIFAR-100-LT with 400 epochs. This experiments conducted on ResNet-32 architecture on CIFAR-100-LT with different imbalance ratios. $\dagger$ represents the performance from each original paper \cite{zhu2022balanced, li2022nested}.}
% \label{tab:cifar_other}
% \centering
% \resizebox{0.4\columnwidth}{!}{
% % \begin{tabular}{lccc}g
% % \thickhline

% % \multirow{2}{*}{Algorithm}  &  \multicolumn{3}{c}{CIFAR-100} \\ \cline{2-4} 
% % \begin{tabular}{l||ccc|ccc}

% \begin{tabular}{p{0.3\textwidth}||>
% {\centering}p{0.08\textwidth}>
% {\centering\arraybackslash}p{0.08\textwidth}}
% \thickhline
% \multirow{2}{*}{Algorithm} 
% & \multicolumn{2}{c}{Imbalance Ratio} \\
% \cline{2-3} 

%                             & 100 & 50 \\ \hline
% % BS~\cite{park2022majority}$^\dagger$
% %                             & $50.0$     & $53.0$    & $60.2$ & -     & -    & - \\
% PaCo~\cite{cui2021parametric}$^\dagger$                        
%                             & $52.0$     & $56.0$      \\
% BCL~\cite{zhu2022balanced}$^\dagger$
%                             & $52.6$ & $57.2$  \\
% % LTR-WB\cite{alshammari2022long}$^\star$
% %                             & $53.4$     & $57.7$    & $68.7$  \\
% % NCL (single)~\cite{li2022nested}$^\dagger$
% %                             & $53.3$     & $56.8$    & - \\
% NCL~\cite{li2022nested}$^\dagger$
%                             & $\underline{54.2}$ & $\underline{58.2}$   \\ \hline
% % \rowcolor[HTML]{EFEFEF} 
% \rowcolor{LightCyan} 
% BCL + CUDA     
%                             & $53.5$     & $57.4$   \\
% % \rowcolor[HTML]{EFEFEF}
% \rowcolor{LightCyan} 
% NCL + CUDA     
%                             & $\mathbf{54.8}$     & $\mathbf{59.6}$   \\ \thickhline

% \end{tabular}
% }
% \end{minipage}
% \end{table}



% % \begin{table}[t!]
% % \begin{minipage}[b]{1.0\linewidth}
% % \caption{Validation accuracy on CIFAR-100-LT with 400 epochs. This experiments conducted on ResNet-32 architecture on CIFAR-100-LT with different imbalance ratios. $\dagger$ represents the performance from each original paper \cite{zhu2022balanced, li2022nested}.}
% % \label{tab:cifar_other}
% % \centering
% % \resizebox{0.5\columnwidth}{!}{
% % % \begin{tabular}{lccc}g
% % % \thickhline

% % % \multirow{2}{*}{Algorithm}  &  \multicolumn{3}{c}{CIFAR-100} \\ \cline{2-4} 
% % % \begin{tabular}{l||ccc|ccc}

% % \begin{tabular}{p{0.3\textwidth}||>
% % {\centering}p{0.06\textwidth}>
% % {\centering}p{0.06\textwidth}|>
% % {\centering}p{0.06\textwidth}>
% % {\centering}p{0.06\textwidth}>
% % {\centering\arraybackslash}p{0.06\textwidth}}
% % \thickhline
% % \multirow{2}{*}{Algorithm} 
% % & \multicolumn{2}{c|}{IR} 
% % & \multicolumn{3}{c}{Statistics (IR 100)} \\
% % \cline{2-3} \cline{4-6}

% %                             & 100 & 50 &  Many & Med & Few \\ \hline
% % % BS~\cite{park2022majority}$^\dagger$
% % %                             & $50.0$     & $53.0$    & $60.2$ & -     & -    & - \\
% % PaCo~\cite{cui2021parametric}$^\dagger$                        
% %                             & $52.0$     & $56.0$     & -     & -    & - \\
% % BCL~\cite{zhu2022balanced}$^\dagger$
% %                             & $53.9$ & -  & $69.7$ & $53.8$ & $35.5$ \\
% % % LTR-WB\cite{alshammari2022long}$^\star$
% % %                             & $53.4$     & $57.7$    & $68.7$  \\
% % % NCL (single)~\cite{li2022nested}$^\dagger$
% % %                             & $53.3$     & $56.8$    & - \\
% % NCL~\cite{li2022nested}$^\dagger$
% %                             & $54.2$ & $58.2$  & $68.3$ & $55.0$ & $38.2$ \\ \hline
% % \rowcolor[HTML]{EFEFEF} 
% % BCL + CUDA     
% %                             & $00.0$     & $00.0$    & $00.0$     & $00.0$    & $00.0$ \\
% % \rowcolor[HTML]{EFEFEF} 
% % NCL + CUDA     
% %                             & $\mathbf{54.8}$     & $00.0$    & $70.3$     & $56.5$    & $35.2$ \\ \thickhline

% % \end{tabular}
% % }
% % \end{minipage}
% % \end{table}


==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/tab/cifar_200ep.tex <==
% \begin{table}[t!]
% \begin{minipage}[b]{1.0\linewidth}
% \caption{Validation accuracy on CIFAR-100-LT dataset. This experiments conducted on ResNet-32 architecture on CIFAR-100-LT with different imbalance ratios. $^\dagger$ are from \citet{park2022majority} and $^\ddagger$ are from the original work\,\cite{kim2020m2m}.}
% \label{tab:cifar_200ep}
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{l||ccc|cccc|cccc}
% \thickhline
% \multirow{2}{*}{Algorithm} 
% & \multicolumn{3}{c|}{CIFAR-100-LT (IR)} 
% & \multicolumn{4}{c|}{ImageNet-LT} & \multicolumn{4}{c}{iNaturalist 2018} \\
% \cline{2-4} \cline{5-8} \cline{9-12}

%                             & 100 & 50 & 10 
%                             & Many & Med & Few & All & Many & Med & Few & All \\ \hline
% CE                          & $38.7$    & $43.4$    & $56.5$ 
%                             & $64.0$    & $33.8$    & $5.8$    & $41.6$ 
%                             & $73.9$    & $63.5$    & $55.5$    & $61.0$ \\
% CE-DRW
%                             & $41.4$    & $45.5$    & $57.8$ 
%                             & $61.7$    & $47.3$    & $28.8$    & $50.1$ 
%                             & -         & -         & -         & - \\
% LDAM-DRW
%                             & $42.5$    & $47.4$    & $57.6$ 
%                             & $60.4$    & $46.9$    & $30.7$    & $49.8$ 
%                             & -         & -         & -         & $66.1$ \\
% BBN$^\dagger$
%                             & $42.6$     & $47.1$    & $59.2$ 
%                             & -         & -         & -         & -
%                             & -         & -         & -         & $69.6$ \\
% M2m + CE$^\ddagger$
%                             & $42.9$     & -         & $58.2$ 
%                             & -         & -         & -         & -
%                             & -         & -         & -         & - \\
% M2m + LDAM$^\ddagger$
%                             & $43.5$     & -         & $57.6$ 
%                             & -         & -         & -         & -
%                             & -         & -         & -         & - \\
% IB Loss$^\dagger$
%                             & $45.0$     & $48.9$    & $61.6$ 
%                             & -         & -         & -         & -
%                             & -         & -         & -         & - \\
% Balanced Softmax$^\dagger$
%                             & $45.7$     & $50.1$    & $61.0$ 
%                             & $60.9$    & $48.8$    & $32.1$    & $51.0$ 
%                             & $70.0$    & $70.2$    & $69.2$    & $70.0$ \\
% Balanced Softmax
%                             & $41.6$     & $46.9$   & $58.3$ 
%                             & -         & -         & -         & -
%                             & -         & -         & -         & - \\
% LADE$^\dagger$
%                             & $45.4$     & $50.5$    & $61.7$ 
%                             & -         & -         & -         & -
%                             & -         & -         & -         & $70.0$ \\
% Remix-DRW$^\dagger$
%                             & $45.8$     & $49.5$    & $59.2$ 
%                             & -         & -         & -         & -
%                             & -         & -         & -         & $70.5$ \\
% MisLAS$^\dagger$
%                             & $47.0$     & $52.3$    & $63.2$ 
%                             & $61.7$    & $51.3$    & $35.8$    & $52.7$ 
%                             & $73.2$    & $72.4$    & $70.4$    & $71.6$ \\
% RIDE (3 experts)$^\dagger$
%                             & $48.6$    & $51.4$    & $59.8$ 
%                             & $66.2$    & $51.7$    & $34.9$    & $54.9$ 
%                             & $70.9$    & $72.4$    & $73.1$    & $72.6$ \\
% RIDE (3 experts)
%                             & $49.7$    & $52.7$    & $60.2$ 
%                             & -         & -         & -         & -
%                             & -         & -         & -         & - \\
% CMO + RIDE$^\dagger$
%                             & $50.0$    & $53.0$    & $60.2$ 
%                             & $66.4$    & $53.9$    & $35.6$    & $56.2$ 
%                             & $68.7$    & $72.6$    & $73.1$    & $72.8$ \\
% CMO + RIDE
%                             & $49.9$    & $53.0$    & $58.9$ 
%                             & -         & -         & -         & -
%                             & -         & -         & -         & - \\
% BCL$^\star$
%                             & $51.9$    & $56.6$    & $64.9$ 
%                             & -         & -         & -         & -
%                             & -         & -         & -         & - \\
% NCL
%                             & $00.0$    & $00.0$    & $00.0$ 
%                             & -         & -         & -         & -
%                             & -         & -         & -         & - \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% CE + CUDA                   & $42.1$    & $47.2$    & $59.6$ 
%                             & -         & -         & -         & -
%                             & -         & -         & -         & - \\
% \rowcolor[HTML]{EFEFEF} 
% CE-DRW + CUDA               & $47.0$    & $52.4$    & $61.6$ 
%                             & -         & -         & -         & -
%                             & -         & -         & -         & - \\
% \rowcolor[HTML]{EFEFEF} 
% LDAM-DRW + CUDA             & $47.6$    & $51.1$    & $58.4$ 
%                             & -         & -         & -         & -
%                             & -         & -         & -         & - \\
% \rowcolor[HTML]{EFEFEF} 
% BS + CUDA                   & $47.6$    & $52.1$    & $61.7$ 
%                             & -         & -         & -         & -
%                             & -         & -         & -         & - \\
% \rowcolor[HTML]{EFEFEF} 
% RIDE (3 experts) + CUDA     & $50.8$    & $53.7$    & $60.2$  
%                             & -         & -         & -         & -
%                             & -         & -         & -         & - \\
% \rowcolor[HTML]{EFEFEF} 
% NCL + CUDA     
%                             & $52.4$    & $00.0$    & $00.0$
%                             & -         & -         & -         & -
%                             & -         & -         & -         & - \\
% \thickhline
% \end{tabular}}
% \end{minipage}
% \end{table}

\begin{table}[t!]
\begin{minipage}[b]{1.0\linewidth}
\caption{Validation accuracy on CIFAR-100-LT dataset. $\dagger$ are from \citet{park2022majority} and $\ddagger$, $   \star$ are from the original papers~\cite{kim2020m2m, zhu2022balanced}. Other results are from our implementation. We format the first and second best results as \textbf{bold} and \underline{underline }. We report the average results of three random trials.}
\label{tab:cifar_200ep}
\centering
\resizebox{0.85\columnwidth}{!}{
% \begin{tabular}{l||ccc|ccc}
\begin{tabular}{p{0.43\textwidth}||>
{\centering}p{0.09\textwidth}>
{\centering}p{0.09\textwidth}>
{\centering}p{0.09\textwidth}|>
{\centering}p{0.09\textwidth}>
{\centering}p{0.09\textwidth}>
{\centering\arraybackslash}p{0.09\textwidth}}
\thickhline
% \toprule
\multirow{2}{*}{Algorithm} 
& \multicolumn{3}{c|}{Imbalance Ratio (IR)} 
& \multicolumn{3}{c}{Statistics (IR 100)} \\
\cline{2-4} \cline{5-7}
% \cmidrule{2-7}

                            & 100 & 50 & 10 
                            & Many & Med & Few \\ \hline
CE                          & $38.7_{\rebut{\pm 0.4}}$    & $43.4_{\rebut{\pm 0.3}}$    & $56.5_{\rebut{\pm 0.6}}$ 
                            & $66.2_{\rebut{\pm 0.5}}$    & $37.3_{\rebut{\pm 0.6}}$    & $8.2_{\rebut{\pm 0.3}}$   \\ 
CE + CMO~\cite{park2022majority}
                            & $42.0_{\rebut{\pm 0.4}}$          & $47.0_{\rebut{\pm 0.5}}$         & $60.0_{\rebut{\pm 0.4}}$ 
                            & $69.1_{\rebut{\pm 0.4}}$          & $41.2_{\rebut{\pm 0.6}}$         & $11.3_{\rebut{\pm 0.7}}$  \\
\rowcolor{LightCyan} 
CE + CUDA                   & $42.7_{\rebut{\pm 0.4}}$    & $47.2_{\rebut{\pm 0.4}}$    & $59.6_{\rebut{\pm 0.4}}$ 
                            & $\mathbf{71.6_{\rebut{\pm 0.6}}}$    & $42.3_{\rebut{\pm 0.3}}$    & $9.4_{\rebut{\pm 0.7}}$  \\
\rowcolor{LightCyan} 
CE + CMO + CUDA
                            & $43.5_{\rebut{\pm 0.5}}$     & $48.7_{\rebut{\pm 0.6}}$    & $60.0_{\rebut{\pm 0.3}}$ 
                            & $70.0_{\rebut{\pm 0.7}}$     & $43.4_{\rebut{\pm 0.5}}$    & $12.7_{\rebut{\pm 0.8}}$  \\\hline
CE-DRW~\citep{cao2019learning}
                            & $41.4_{\rebut{\pm 0.2}}$    & $45.5_{\rebut{\pm 0.6}}$    & $57.8_{\rebut{\pm 0.6}}$ 
                            & $62.8_{\rebut{\pm 0.5}}$    & $41.7_{\rebut{\pm 0.7}}$    & $16.1_{\rebut{\pm 0.4}}$  \\
CE-DRW + Remix~\citep{chou2020remix}$^\dagger$
                            & $45.8$     & $49.5$    & $59.2$ 
                            & -         & -         & -  \\ 
% \rowcolor[HTML]{EFEFEF} 
\rowcolor{LightCyan} 
CE-DRW + CUDA               & $47.7_{\rebut{\pm 0.4}}$ & $52.4_{\rebut{\pm 0.5}}$    & $61.6_{\rebut{\pm 0.5}}$ 
                            & $64.3_{\rebut{\pm 0.4}}$    & $49.2_{\rebut{\pm 0.6}}$    & $26.7_{\rebut{\pm 0.6}}$  \\ \hline

LDAM-DRW~\citep{cao2019learning}
                            & $42.5_{\rebut{\pm 0.2}}$    & $47.4_{\rebut{\pm 0.5}}$    & $57.6_{\rebut{\pm 0.1}}$ 
                            & $62.8_{\rebut{\pm 0.5}}$    & $42.3_{\rebut{\pm 0.6}}$    & $19.0_{\rebut{\pm 0.7}}$  \\ 
LDAM + M2m~\cite{kim2020m2m}$^\ddagger$
                            & $43.5$     & -         & $57.6$ 
                            & -          & -         & -  \\ 

% \rowcolor[HTML]{EFEFEF} 
\rowcolor{LightCyan} 
LDAM-DRW + CUDA
                            & $47.6_{\rebut{\pm 0.7}}$    & $51.1_{\rebut{\pm 0.4}}$    & $58.4_{\rebut{\pm 0.1}}$ 
                            & $67.3_{\rebut{\pm 0.6}}$    & $50.4_{\rebut{\pm 0.5}}$    & $21.4_{\rebut{\pm 0.2}}$ \\ \hline
BS~\citep{ren2020balanced}
                            & $43.3_{\rebut{\pm 0.4}}$     & $46.9_{\rebut{\pm 0.2}}$   & $58.3_{\rebut{\pm 0.4}}$ 
                            & $61.6_{\rebut{\pm 0.8}}$     & $42.3_{\rebut{\pm 0.5}}$   & $23.0_{\rebut{\pm 0.4}}$  \\
% \rowcolor[HTML]{EFEFEF} 
\rowcolor{LightCyan} 
BS + CUDA                   & $47.7_{\rebut{\pm 0.3}}$    & $52.1_{\rebut{\pm 0.4}}$    & $61.7_{\rebut{\pm 0.5}}$ 
                            & $63.3_{\rebut{\pm 0.4}}$    & $48.4_{\rebut{\pm 0.4}}$    & $28.7_{\rebut{\pm 0.5}}$  \\ \hline
RIDE (3 experts)~\citep{wang2021longtailed}$^\dagger$
                            & $48.6$    & $51.4$    & $59.8$ 
                            & -         & -         & -  \\
RIDE (3 experts)
                            & $49.7_{\rebut{\pm 0.2}}$    & $52.7_{\rebut{\pm 0.1}}$    & $60.2_{\rebut{\pm 0.2}}$ 
                            & $67.7_{\rebut{\pm 0.6}}$    & $51.5_{\rebut{\pm 0.5}}$    & $26.7_{\rebut{\pm 0.6}}$   \\  
RIDE + CMO~\citep{park2022majority}$^\dagger$
                            & $50.0$    & $53.0$    & $60.2$ 
                            & -         & -         & -  \\
RIDE + CMO
                            & $49.9_{\rebut{\pm 0.1}}$    & $53.0_{\rebut{\pm 0.1}}$    & $58.9_{\rebut{\pm 0.3}}$ 
                            & $67.3_{\rebut{\pm 0.3}}$    & $51.3_{\rebut{\pm 0.6}}$    & $28.1_{\rebut{\pm 0.4}}$  \\ 
\rowcolor{LightCyan} 
RIDE (3 experts) + CUDA     & $50.7_{\rebut{\pm 0.2}}$    & $53.7_{\rebut{\pm 0.4}}$    & $60.2_{\rebut{\pm 0.1}}$  
                            & $\underline{69.2_{\rebut{\pm 0.3}}}$    & $52.8_{\rebut{\pm 0.2}}$    & $27.3_{\rebut{\pm 0.8}}$  \\  \hline
BCL~\cite{zhu2022balanced}$^\star$
                            & $\underline{51.0}$    & $\underline{54.9}$    & $\underline{64.4}$ 
                            & $67.2$    & $\underline{53.1}$    & $\underline{32.9}$  \\
\rowcolor{LightCyan} 
BCL + CUDA     
                            & $\mathbf{52.3_{\rebut{\pm 0.2}}}$    & $\mathbf{56.2_{\rebut{\pm 0.4}}}$    & $\mathbf{64.6_{\rebut{\pm 0.1}}}$
                            & $66.4_{\rebut{\pm 0.2}}$    & $\mathbf{54.2_{\rebut{\pm 0.6}}}$    & $\mathbf{33.9_{\rebut{\pm 0.8}}}$ \\
\thickhline
\end{tabular}}
\end{minipage}
\vspace{-7pt}
\end{table}







==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/tab/curriculum.tex <==

\begin{figure}[!t]
  \centering
  \begin{subfigure}{0.195\linewidth}
          \includegraphics[width=\linewidth]{fig/CE_Heat.pdf}
          \vspace{-16pt}
          \caption{CE}
  \end{subfigure}
%   \hspace{-0.1in}
    \begin{subfigure}{0.195\linewidth}
          \includegraphics[width=\linewidth]{fig/CE-DRW_Heat.pdf}
          \vspace{-16pt}
          \caption{CE-DRW}
  \end{subfigure}
  \begin{subfigure}{0.195\linewidth}
          \includegraphics[width=\linewidth]{fig/LDAM_Heat.pdf}
          \vspace{-16pt}
          \caption{LDAM-DRW}
  \end{subfigure}
%   \hspace{-0.1in}
  \begin{subfigure}{0.195\linewidth}
          \includegraphics[width=\linewidth]{fig/BS_Heat.pdf}
          \vspace{-16pt}
          \caption{BS}
  \end{subfigure}
%   \hspace{-0.1in}
  \begin{subfigure}{0.195\linewidth}
          \includegraphics[width=\linewidth]{fig/RIDE_Heat.pdf}
          \vspace{-16pt}
          \caption{RIDE}
  \end{subfigure}
  \vspace{-7pt}
  \caption{Evolution of LoL score on various algorithms, CE, CE-DRW, LDAM-DRW, BS, and RIDE.  }
  \label{fig:curriculum}
  \vspace{-15pt}
\end{figure}


==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/tab/norm_softmax.tex <==
\vspace{-3pt}
\begin{figure}[!t]
  \centering
  \begin{subfigure}{0.195\linewidth}
        %   \includegraphics[width=\linewidth]{fig/ce_wnorm.pdf}\\
            \includegraphics[width=\linewidth]{fig/CE_stdev.pdf}\\
            \includegraphics[width=\linewidth]{fig/ce_align.pdf}
            \vspace{-15pt}
          \caption{CE}
  \end{subfigure}
  \begin{subfigure}{0.195\linewidth}
        %   \includegraphics[width=\linewidth]{fig/ce-drw_wnorm.pdf}\\
            \includegraphics[width=\linewidth]{fig/CE-DRW_stdev.pdf}\\
            \includegraphics[width=\linewidth]{fig/ce-drw_align.pdf}
            \vspace{-15pt}
          \caption{CE-DRW}
  \end{subfigure}
  \begin{subfigure}{0.195\linewidth}
        %   \includegraphics[width=\linewidth]{fig/ldam-zero_wnorm.pdf}\\
            \includegraphics[width=\linewidth]{fig/LDAM_stdev.pdf}\\
            \includegraphics[width=\linewidth]{fig/ldam-drw_align.pdf}
            \vspace{-15pt}
          \caption{LDAM-DRW}
  \end{subfigure}
  \begin{subfigure}{0.195\linewidth}
            % \includegraphics[width=\linewidth]{fig/bs_wnorm.pdf}\\
            \includegraphics[width=\linewidth]{fig/BS_stdev.pdf}\\
            \includegraphics[width=\linewidth]{fig/bs_align.pdf}
            \vspace{-15pt}
          \caption{BS}
  \end{subfigure}
  \begin{subfigure}{0.195\linewidth}
            % \includegraphics[width=\linewidth]{fig/ride-zero_wnorm.pdf}\\
            \includegraphics[width=\linewidth]{fig/RIDE_stdev.pdf}\\
            \includegraphics[width=\linewidth]{fig/ride_align.pdf}
            \vspace{-15pt}
          \caption{RIDE}
  \end{subfigure}
  \vspace{-7pt}
  \caption{Analysis of how \alg improves long-tailed recognition performance, classifier weight norm (top row) and feature alignment \rebut{gain} (bottom row) of the CIFAR-100-LT validation set. Notably that weight norm and feature alignment represent class-wise weight magnitude of classifier and ability of feature extractor, respectively. The detailed analysis is described in Section~\ref{exp:analysis}.}
  \vspace{-7pt}
  \label{fig:output_analysis}
\end{figure}



% \begin{table}
% \begin{minipage}{0.65\linewidth}
%     \begin{subfigure}{0.32\linewidth}
%           \includegraphics[width=\linewidth]{example-image-golden}
%           \caption{$\gamma$}
%     \end{subfigure}
%     \begin{subfigure}{0.32\linewidth}
%           \includegraphics[width=\linewidth]{example-image-golden}
%           \caption{$n$}
%     \end{subfigure}
%     \begin{subfigure}{0.32\linewidth}
%           \includegraphics[width=\linewidth]{example-image-golden}
%           \caption{$p_{\text{aug}}$}
%     \end{subfigure}
%     \captionof{figure}{Parameter sensitivitiy analysis.}
% \end{minipage}
% \begin{minipage}{0.35\linewidth}
%     \resizebox{1\linewidth}{!}{
%     \begin{tabular}{cc|cccc}
%         \thickhline
%         Curr & $p_{\text{aug}}$ & All & Many & Med & Few \\ \hline
%         & &         $00.0$ & $00.0$ & $00.0$ & $00.0$ \\
%         \cmark & & $00.0$ & $00.0$ & $00.0$ & $00.0$ \\
%          & \cmark& $00.0$ & $00.0$ & $00.0$ & $00.0$ \\
%          \cmark & \cmark& $00.0$ & $00.0$ & $00.0$ & $00.0$ \\
%         \thickhline
%     \end{tabular}
%     }
%     \caption{Ablation study. Curr and $p_{\text{aug}}$ represents curriculum and augmentation probability, respectively.}
% \end{minipage}
% \end{table}

==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/tab/real_world.tex <==

\begin{table}[t!]
\begin{minipage}[b]{1.0\linewidth}
\caption{Validation accuracy on ImageNet-LT and iNaturalist 2018 datasets. $\dagger$ indicates reported results from the \citet{park2022majority} and $\ddagger$ indicates those from the original paper~\cite{kang2019decoupling}. $\star$ means we train the network with the official code in an one-stage RIDE.}
\centering
\resizebox{0.9\columnwidth}{!}{
% \begin{tabular}{l||ccc|c|ccc|c}
\begin{tabular}{p{0.4\textwidth}||>
{\centering}p{0.09\textwidth}>
{\centering}p{0.09\textwidth}>
{\centering}p{0.09\textwidth}|>
{\centering}p{0.09\textwidth}|>
{\centering}p{0.09\textwidth}>
{\centering}p{0.09\textwidth}>
{\centering}p{0.09\textwidth}|>
{\centering\arraybackslash}p{0.09\textwidth}}
\thickhline
\multirow{2}{*}{Algorithm} 
&  \multicolumn{4}{c|}{ImageNet-LT}  
& \multicolumn{4}{c}{iNaturalist 2018} \\
\cline{2-5} \cline{6-9}
                            & Many & Med & Few & All
                            & Many & Med & Few & All\\ \hline
CE$^\dagger$                          
                            & $64.0$    & $33.8$    & $5.8$    & $41.6$ 
                            & $73.9$    & $63.5$    & $55.5$    &  $61.0$ \\
\rowcolor{LightCyan} 
CE + CUDA                   
                            & $\rebut{\mathbf{67.2}_{\pm 0.1}}$    & $\rebut{47.0_{\pm 0.2}}$    & $\rebut{13.5_{\pm 0.3}}$    & $\rebut{47.3_{\pm 0.2}}$ 
                            & $\mathbf{74.6}_{\rebut{\pm 0.3}}$    & $\rebut{64.9_{\pm 0.1}}$    & $57.2_{\rebut{\pm 0.1}}$ & $62.5_{\rebut{\pm 0.2}}$ \\ \hline
CE-DRW~\cite{cao2019learning}
                            & $61.7_{\rebut{\pm 0.1}}$    & $\rebut{47.1_{\pm 0.3}}$    & $\rebut{29.0_{\pm 0.3}}$    & $50.1_{\rebut{\pm 0.1}}$ 
                            & $68.2_{\rebut{\pm 0.2}}$    & $67.3_{\rebut{\pm 0.2}}$    & $66.4_{\rebut{\pm 0.1}}$    & $67.0_{\rebut{\pm 0.1}}$ \\
\rowcolor{LightCyan} 
CE-DRW + CUDA               
                            & $\rebut{61.8_{\pm 0.1}}$    & $\rebut{48.3_{\pm 0.1}}$    & $30.3_{\rebut{\pm 0.2}}$    & $\rebut{51.0_{\pm 0.1}}$ 
                            & $68.8_{\rebut{\pm 0.1}}$    & $\rebut{68.1_{\pm 0.3}}$    & $\rebut{66.6_{\pm 0.2}}$    & $\rebut{67.5_{{\pm 0.1}}}$ \\ \hline
LWS~\cite{kang2019decoupling}$^\ddagger$
                            & $57.1$    & $45.2$    & $29.3$    & $47.7$ 
                            & $65.0$    & $66.3$    & $65.5$    & $65.9$ \\
cRT~\cite{kang2019decoupling}$^\ddagger$
                            & $58.8$    & $44.0$    & $26.1$    & $47.3$ 
                            & $69.0$    & $66.0$    & $63.2$    & $65.2$ \\
\rowcolor{LightCyan}
cRT + CUDA
                            & $62.3_{\rebut{\pm 0.1}}$    & $\rebut{47.2_{\pm 0.2}}$    & $\rebut{28.4_{\pm 0.5}}$    & $50.2_{\rebut{\pm 0.2}}$
                            & $68.2_{\rebut{\pm 0.1}}$    & $\rebut{67.8_{\pm 0.2}}$    & $66.4_{\rebut{\pm 0.1}}$    & $67.3_{\rebut{\pm 0.1}}$ \\ \hline
LDAM-DRW~\cite{cao2019learning}$^\dagger$
                            & $60.4$    & $46.9$    & $30.7$    & $49.8$ 
                            & -         & -         & -         & $66.1$ \\
\rowcolor{LightCyan} 
LDAM-DRW + CUDA             
                            & $63.1_{\rebut{\pm 0.1}}$    & $\rebut{48.0_{\pm 0.3}}$    & $\rebut{31.1_{\pm 0.2}}$    & $\rebut{51.4_{\pm 0.1}}$ 
                            & $\rebut{67.8_{\pm 0.2}}$    & $\rebut{67.6_{\pm 0.2}}$    & $\rebut{66.7_{\pm 0.3}}$    & $\rebut{67.2_{\pm 0.2}}$ \\ \hline
BS~\cite{ren2020balanced}
                            & $\rebut{61.1_{\pm 0.2}}$    & $\rebut{48.5_{\pm 0.2}}$    & $\rebut{31.8_{\pm 0.4}}$    & $\rebut{50.9_{\pm 0.1}}$ 
                            & $\rebut{65.5_{\pm 0.2}}$    & $\rebut{67.5_{\pm 0.1}}$    & $67.5_{\rebut{\pm 0.1}}$    & $\rebut{67.2_{\pm 0.2}}$ \\
\rowcolor{LightCyan} 
BS + CUDA                   
                            & $\rebut{61.9_{\pm 0.1}}$    & $\rebut{49.2_{\pm 0.0}}$    & $\rebut{32.3_{\pm 0.4}}$    & $\rebut{51.6_{\pm 0.1}}$ 
                            & $67.6_{\rebut{\pm 0.1}}$    & $\rebut{68.3_{\pm 0.1}}$    & $68.3_{\rebut{\pm 0.1}}$    & $68.2_{\rebut{\pm 0.1}}$ \\ \hline
RIDE (3 experts)~\cite{wang2021longtailed}$^\star$
                            & $\rebut{64.8_{\pm 0.1}}$    & $\rebut{50.8_{\pm 0.2}}$    & $\rebut{34.6_{\pm 0.2}}$    & $53.6_{\rebut{\pm 0.1}}$ 
                            & $70.4_{\rebut{\pm 0.1}}$    & $71.8_{\rebut{\pm 0.1}}$    & $\rebut{71.7_{\pm 0.1}}$    & $71.6_{\rebut{\pm 0.1}}$ \\
RIDE + CMO~\cite{park2022majority}$^\star$
                            & $65.6$    & $50.6$    & $34.8$    & $54.0$ 
                            & $68.0$    & $70.6$    & $\underline{72.0}$    & $70.9$ \\
\rowcolor{LightCyan} 
RIDE (3 experts) + CUDA$^\star$     
                            & $\rebut{65.9_{\pm 0.1}}$    & $51.7_{\rebut{\pm 0.2}}$    & $\rebut{34.9_{\pm 0.2}}$    & $54.7_{\rebut{\pm 0.1}}$ 
                            & $\rebut{70.7_{\pm 0.2}}$    & $\rebut{\underline{72.5}_{\pm 0.1}}$ & $\mathbf{72.7}_{\rebut{\pm 0.2}}$    & $\mathbf{72.4}_{\rebut{\pm 0.2}}$ \\ \hline
BCL~\cite{zhu2022balanced}
                            & $65.3_{\rebut{\pm 0.2}}$    & $\underline{53.5}_{\rebut{\pm 0.2}}$    & $\underline{36.3}_{\rebut{\pm 0.3}}$    & $\underline{55.6}_{\rebut{\pm 0.2}}$
                            & $\rebut{69.5_{\pm 0.1}}$    & $72.4_{\rebut{\pm 0.2}}$    & $\rebut{71.7_{\pm 0.1}}$    & $71.8_{\rebut{\pm 0.1}}$ \\
\rowcolor{LightCyan}
BCL + CUDA     
                            & $\underline{66.8}_{\rebut{\pm 0.1}}$    & $\mathbf{53.9}_{\rebut{\pm 0.3}}$    & $\mathbf{36.6}_{\rebut{\pm 0.2}}$    & $\mathbf{56.3}_{\rebut{\pm 0.1}}$ 
                            & $\rebut{\underline{70.9}_{\pm 0.2}}$    & $\rebut{\mathbf{72.8}_{\pm 0.1}}$    & $\underline{72.0}_{\rebut{\pm 0.1}}$    & $\rebut{\underline{72.3}_{\pm 0.1}}$ \\
\thickhline
\end{tabular}
}\label{tab:in_inat}
\end{minipage}
\end{table}

==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/tab/rebuttal/augment_number.tex <==
\begin{table}[ht]
\centering
\caption{\rebut{The performance comparison of \alg with different number ($K$) of predefined augmentation operations.}}\label{tab:augment_number}
\resizebox{0.8\columnwidth}{!}{
\rebut{
\begin{tabular}{l|c|ccccc}
\thickhline
                                                & Category & CE & CE-DRW & LDAM-DRW & BS & RIDE \\ \midrule
\multirow{4}{*}{Vanilla (w/o augmentation)} & Many                         & 66.2                   & 62.8                       & 62.8                         & 61.6                   & 67.7                     \\
                                                & Med                          & 37.3                   & 41.7                       & 42.3                         & 42.3                   & 51.5                     \\
                                                & Few                          & 8.2                    & 16.2                       & 19.0                         & 23.0                   & 26.7                     \\
                                                & All                          & 38.7                   & 41.4                       & 42.5                         & 43.3                   & 49.7                     \\  \midrule
\multirow{4}{*}{Random Selection (K=10)}                      & Many                         & 70.8                   & 62.3                       & 65.2                         & 62.6                   & 68.5                     \\
                                                & Med                          & 40.4                   & 49.0                       & 49.2                         & 46.9                   & 52.0                     \\
                                                & Few                          & 9.0                    & 26.7                       & 21.6                         & 27.3                   & 27.1                     \\
                                                & All                          & 41.6                   & 47.0                       & 46.5                         & 46.5                   & 50.3                     \\  \midrule
\multirow{4}{*}{RandAugment (K=14)}                    & Many                         & 70.3                   & 63.5                       & 65.4                         & 62.9                   & 68.5                     \\
                                                & Med                          & 40.7                   & 49.1                       & 50.6                         & 48.1                   & 52.3                     \\
                                                & Few                          & 9.6                    & 26.0                       & 21.6                         & 28.7                   & 27.0                     \\
                                                & All                          & 41.8                   & 47.2                       & 47.1                         & 47.5                   & 50.4                     \\  \midrule
\multirow{4}{*}{Ours (K=22)}                    & Many                         & 71.6                   & 64.3                       & 67.3                         & 63.3                   & 69.2                     \\
                                                & Med                          & 42.3                   & 49.2                       & 50.4                         & 48.4                   & 52.8                     \\
                                                & Few                          & 9.4                    & 26.7                       & 21.4                         & 28.7                   & 27.3                     \\
                                                & All                          & 42.7                   & 47.7                       & 47.6                         & 47.7                   & 50.7   \\
\thickhline
\end{tabular}}}
\end{table}

==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/tab/rebuttal/classifier_norm.tex <==
\begin{table}[ht]
\centering
\caption{\rebut{The comparison of variance of L1 norm for class-wise linear classifier between various augmentation strategy (vanilla, AutoAugment\,\cite{cubuk2019autoaugment}, and \alg).}}\label{tab:classifier_norm}
\resizebox{1.0\columnwidth}{!}{
\rebut{
\begin{tabular}{l|ccccccccccc}
\thickhline
Augment / Epoch & 0 & 20 & 40 & 60 & 80 & 100 & 120 & 140 & 160 & 180 & 200 \\ \midrule
Vanilla (w/o Augment)         & 0.826                 & 3.018                  & 3.448                  & 3.470                   & 3.342                  & 3.202                   & 3.093                   & 3.104                   & 3.044                   & 2.967                   & 2.967                   \\
AutoAugment         & 0.819                 & 2.700                    & 3.149                  & 3.065                  & 2.958                  & 2.908                   & 2.810                    & 2.723                   & 2.646                   & 2.527                   & 2.526                   \\
\alg            & 0.821                 & 2.651                  & 2.892                  & 2.708                  & 2.502                  & 2.444                   & 2.393                   & 2.364                   & 2.297                   & 2.182                   & 2.182         \\
\thickhline
\end{tabular}}}
\end{table}

==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/tab/rebuttal/classwise.tex <==
\begin{table}[ht]
\centering
\caption{\rebut{The performance comparison between different augmentation strategy on CIFAR-100-LT with imbalance ratio 100. Note that values in parentheses are differences of \alg w/o class-wise with vanilla (vanilla - \alg w/o class-wise) or \alg (\alg - \alg w/o class-wise).}}\label{tab:class-wise}
\resizebox{0.8\columnwidth}{!}{
\rebut{
\begin{tabular}{l|c|ccccc}
\thickhline
                                     & Category & CE & CE-DRW &  LDAM-DRW & BS & RIDE \\ \midrule
\multirow{4}{*}{\alg w/o class-wise} & Many     & 69.0                   & 62.7                       & 65.2                         & 62.2                   & 67.7                     \\
                                     & Med      & 38.7                   & 47.3                       & 47.6                         & 44.7                   & 52.2                     \\
                                     & Few      & 6.7                    & 23.5                       & 20.7                         & 25.5                   & 26.4                     \\
                                     & All      & 39.7                   & 45.5                       & 45.7                         & 44.9                   & 49.9                     \\ \midrule
\multirow{4}{*}{Vanilla}             & Many     & 66.2 (-2.8)            & 62.8 (+0.1)                & 62.8 (-2.4)                  & 61.6 (-0.6)            & 67.7 (+0.0)              \\
                                     & Med      & 37.3 (-1.4)            & 41.7 (-5.6)                & 42.3 (-5.3)                  & 42.3 (-2.4)            & 51.5 (-0.7)              \\
                                     & Few      & 8.2 (+1.5)             & 16.2 (-7.3)                & 19.0 (-1.7)                  & 23.0 (-2.5)            & 26.7 (+0.3)              \\
                                     & All      & 38.7 (-1.0)            & 41.4 (-4.1)                 & 42.5 (-3.2)                  & 43.3 (-1.6)            & 49.7 (-0.2)              \\ \midrule
\multirow{4}{*}{\alg (Ours)}         & Many     & 71.6 (+2.6)            & 64.3 (+1.6)                & 67.3 (+2.1)                  & 63.3 (+1.1)            & 69.2 (+1.5)              \\
                                     & Med      & 42.3 (+3.6)            & 49.2 (+1.9)                & 50.4 (+2.8)                  & 48.4 (+3.7)            & 52.8 (+0.6)              \\
                                     & Few      & 9.4 (+2.7)             & 26.7 (+3.2)                & 21.4 (+0.7)                  & 28.7 (+3.2)            & 27.3 (+0.9)              \\
                                     & All      & 42.7 (+3.0)            & 47.7 (+2.2)                & 47.6 (+1.9)                  & 47.7 (+2.8)            & 50.7 (+0.8)             \\
\thickhline
\end{tabular}}}
\end{table}

==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/tab/rebuttal/finding.tex <==
\begin{table}[ht]
\centering
\caption{\rebut{The performance comparison between different augmentation strength on major (class indices 0-49) and minor (class indices 50-99) categories. }}\label{tab:findings}
\resizebox{1.0\columnwidth}{!}{
\rebut{
\begin{tabular}{l|c|cccc|l|c|cccc}
\thickhline
                          & (major, minor) & Many & Med & Few & All &   & (major, minor) & Many & Med & Few & All \\ \midrule
\multirow{4}{*}{CE}       & 0,0            & 66.2                     & 37.3                    & 8.2                     & 38.7                    & \multirow{4}{*}{CE-DRW} & 0,0                  & 62.8                     & 41.7                    & 16.2                    & 41.4                    \\
                          & 0,4            & 69.7                     & 30.4                    & 2.3                     & 35.7                    &                         & 0,4                  & 65.9                     & 37.2                    & 10.6                    & 39.3                    \\
                          & 4,0            & 60.9                     & 39.3                    & 12.8                    & 38.9                    &                         & 4,0                  & 49.3                     & 45.2                    & 28.3                    & 41.6                    \\
                          & 4,4            & 67.0                     & 34.5                    & 4.7                     & 37.0                    &                         & 4,4                  & 56.6                     & 46.6                    & 24.6                    & 43.5                    \\ \midrule
\multirow{4}{*}{LDAM-DRW} & 0,0            & 62.8                     & 42.3                    & 19.0                    & 42.5                    & \multirow{4}{*}{BS}     & 0,0                  & 61.6                     & 42.3                    & 23.0                    & 43.3                    \\
                          & 0,4            & 70.1                     & 34.3                    & 6.4                     & 38.5                    &                         & 0,4                  & 66.9                     & 37.9                    & 10.8                    & 39.9                    \\
                          & 4,0            & 52.3                     & 42.0                    & 27.7                    & 41.3                    &                         & 4,0                  & 48.7                     & 42.5                    & 28.7                    & 40.5                    \\
                          & 4,4            & 61.1                     & 43.4                    & 17.3                    & 41.8                    &                         & 4,4                  & 56.3                     & 44.2                    & 23.0                    & 42.1                    \\ \midrule
\multirow{4}{*}{RIDE}     & 0,0            & 67.7                     & 51.5                    & 26.7                    & 49.7                    &  \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    \\
                          & 0,4            & 70.5                     & 36.8                    & 7.7                     & 39.9                    & \multicolumn{1}{r}{}    & \multicolumn{1}{r}{} & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    \\
                          & 4,0            & 56.6                     & 44.5                    & 27.2                    & 43.6                    & \multicolumn{1}{r}{}    & \multicolumn{1}{r}{} & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    \\
                          & 4,4            & 62.3                     & 44.5                    & 21.6                    & 43.9                    & \multicolumn{1}{r}{}    & \multicolumn{1}{r}{} & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}   \\
\thickhline
\end{tabular}}}
\end{table}

==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/tab/rebuttal/fix_order.tex <==
\begin{table}[ht]
\centering
\caption{\rebut{The performance comparison of \alg with random order (Ours) and fixed order of augmentation operations. Note that the values in parentheses are differences between \alg and \alg with fixed augmentation order (Random order $-$ Fixed order).}}\label{tab:fix_order}
\resizebox{1.0\columnwidth}{!}{
\rebut{
\begin{tabular}{l|c|ccccc}
\thickhline
                             & Category & CE & CE-DRW & LDAM-DRW & BS & RIDE \\ \midrule
\multirow{4}{*}{Random order (Ours)} & Many     & 71.6                   & 64.3                       & 67.3                         & 63.3                   & 69.2                     \\
                             & Med      & 42.3                   & 49.2                       & 50.4                         & 48.4                   & 52.8                     \\
                             & Few      & 9.4                    & 26.7                       & 21.4                         & 28.7                   & 27.3                     \\
                             & All      & 42.7                   & 47.7                       & 47.6                         & 47.7                   & 50.7                     \\ \midrule
\multirow{4}{*}{Fixed order}   & Many     & 70.5 (-1.1)            & 62.8 (-1.5)                & 66.9 (-0.4)                  & 62.5 (-0.8)            & 68.2 (-1.0)              \\
                             & Med      & 43.0 (+0.7)            & 50.2 (+1.0)                & 49.7 (-0.7)                  & 48.3 (-0.1)            & 53.5 (+0.7)              \\
                             & Few      & 9.0 (-0.4)             & 27 (+0.3)                  & 21.9 (+0.5)                  & 29.6 (+0.9)            & 26.9 (-0.4)              \\
                             & All      & 42.4 (-0.3)            & 47.7 (+0.0)                & 47.4 (-0.2)                  & 47.7 (+0.0)            & 50.5 (-0.2)   \\
\thickhline
\end{tabular}}}
\end{table}

==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/tab/rebuttal/lol_dynamics.tex <==
\begin{table}[ht]
\centering
\caption{\rebut{The averaged LoL score of top 10 classes (class indices with 1-10) and bottom classes (class indices with 91-100) for every 20 epochs.}}\label{tab:lol_dynamics}
\resizebox{0.75\columnwidth}{!}{
\rebut{
\begin{tabular}{l|c|cccccccccc}
\thickhline
                          & Class / Epoch & 20 & 40 & 60 & 80 & 100 & 120 & 140 & 160 & 180 & 200 \\ \midrule
\multirow{2}{*}{CE}       & Top 10    & 0.5                    & 0.8                    & 1.7                    & 2                      & 2.6                     & 2.7                     & 3.2                     & 3.2                     & 3.4                     & 3.7                     \\
                          & Bottom 10 & 0.0                    & 0.0                    & 0.0                    & 0.0                    & 0.0                     & 0.1                     & 0.0                     & 0.1                     & 0.0                     & 0.1                     \\ \midrule
\multirow{2}{*}{CE-DRW}   & Top 10    & 0.8                    & 1.3                    & 2                      & 2.5                    & 1.6                     & 2.6                     & 1.8                     & 2.6                     & 2.5                     & 2.6                     \\
                          & Bottom 10 & 0.0                    & 0.0                    & 0.0                    & 0.0                    & 0.0                     & 0.1                     & 0.0                     & 0.0                     & 1.2                     & 1.4                     \\ \midrule
\multirow{2}{*}{LDAM-DRW} & Top 10    & 1.8                    & 3.4                    & 3.3                    & 3                      & 3.4                     & 3.2                     & 3.1                     & 3.6                     & 4.1                     & 4.3                     \\
                          & Bottom 10 & 0.0                    & 0.0                    & 0.1                    & 0.0                    & 0.0                     & 0.1                     & 0.0                     & 0.0                     & 1.8                     & 1.4                     \\ \midrule
\multirow{2}{*}{BS}       & Top 10    & 1.1                    & 1.1                    & 1.6                    & 2.4                    & 2.1                     & 2.5                     & 2.5                     & 2.8                     & 3.9                     & 4.0                     \\
                          & Bottom 10 & 0.1                    & 0.1                    & 0.0                    & 0.1                    & 0.6                     & 1.1                     & 1.0                     & 0.7                     & 1.7                     & 1.4                     \\ \midrule
\multirow{2}{*}{RIDE}     & Top 10    & 0.8                    & 1.2                    & 1.6                    & 1.7                    & 2.1                     & 1.8                     & 1.3                     & 1.1                     & 2.5                     & 2.6                     \\
                          & Bottom 10 & 0.0                    & 0.0                    & 0.0                    & 0.0                    & 0.0                     & 0.0                     & 0.0                     & 0.0                     & 0.7                     & 0.8   \\
\thickhline
\end{tabular}}}
\end{table}

==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/tab/rebuttal/lol_score.tex <==
\begin{table}[ht]
\centering
\caption{\rebut{The performance comparison between the scores for determining strength parameter, \citet{sinha2022class} and LoL score (ours). }}\label{tab:lol_score}
\resizebox{0.85\columnwidth}{!}{
\rebut{
\begin{tabular}{l|c|ccccc}
\thickhline
                                  & Category & CE & CE-DRW & LDAM-DRW & BS & RIDE \\ \midrule
\multirow{4}{*}{\citet{sinha2022class}}          & Many     & 68.4                   & 59.7                       & 62.0                         & 59.7                   & 67                       \\
                                  & Med      & 42.5                   & 48.8                       & 48.7                         & 47.0                   & 52.1                     \\
                                  & Few      & 11.6                   & 27.3                       & 25.4                         & 32.0                   & 26.7                     \\
                                  & All      & 42.3                   & 46.1                       & 46.4                         & 46.9                   & 49.6                     \\ \midrule
\multirow{4}{*}{LoL score} & Many     & 71.6                   & 64.3                       & 67.3                         & 63.3                   & 69.2                     \\
                                  & Med      & 42.3                   & 49.2                       & 50.4                         & 48.4                   & 52.8                     \\
                                  & Few      & 9.4                    & 26.7                       & 21.4                         & 28.7                   & 27.3                     \\
                                  & All      & 42.7                   & 47.7                       & 47.6                         & 47.7                   & 50.7    \\
\thickhline
\end{tabular}}}
\end{table}

==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/tab/rebuttal/random_augment.tex <==
\begin{table}[ht]
\centering
\caption{\rebut{The performance comparison between train network with randomly selected five and ten augmentation operations for every iteration and our proposed \alg.}}\label{tab:random_augment}
\resizebox{0.8\columnwidth}{!}{
\rebut{
\begin{tabular}{l|c|ccccc}
\thickhline
                           & Category & CE & CE-DRW & LDAM-DRW & BS & RIDE \\ \midrule
\multirow{4}{*}{Vanilla}   & Many                 & 66.2                   & 62.8                       & 62.8                         & 61.6                   & 67.7                     \\
                           & Med                  & 37.3                   & 41.7                       & 42.3                         & 42.3                   & 51.5                     \\
                           & Few                  & 8.2                    & 16.2                       & 19                           & 23                     & 26.7                     \\
                           & All                  & 38.7                   & 41.4                       & 42.5                         & 43.3                   & 49.7                     \\ \midrule
\multirow{4}{*}{Randomly selected 5 augmentations}  & Many                 & 68.9                   & 56.9                       & 64.2                         & 59.5                   & 64                       \\
                           & Med                  & 35                     & 48.2                       & 42.7                         & 48.2                   & 44.8                     \\
                           & Few                  & 3.7                    & 25.6                       & 16.3                         & 23                     & 20                       \\
                           & All                  & 37.5                   & 44.5                       & 42.3                         & 44.6                   & 44.1                     \\ \midrule
\multirow{4}{*}{Randomly selected 10 augmentations} & Many                 & 61.7                   & 51.2                       & 57.9                         & 54                     & 57.7                     \\
                           & Med                  & 25.7                   & 43.2                       & 34.7                         & 41.2                   & 38.3                     \\
                           & Few                  & 1.3                    & 20.6                       & 12.7                         & 16.8                   & 16.6                     \\
                           & All                  & 31.0                     & 39.2                       & 36.2                         & 38.4                   & 38.6                     \\ \midrule
\multirow{4}{*}{\alg}      & Many                 & 71.6                   & 64.3                       & 67.3                         & 63.3                   & 69.2                     \\
                           & Med                  & 42.3                   & 49.2                       & 50.4                         & 48.4                   & 52.8                     \\
                           & Few                  & 9.4                    & 26.7                       & 21.4                         & 28.7                   & 27.3                     \\
                           & All                  & 42.7                   & 47.7                       & 47.6                         & 47.7                   & 50.7                    \\
\thickhline
\end{tabular}}}
\end{table}

==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/tab/rebuttal/random_sample.tex <==
\begin{table}[ht]
\centering
\caption{\rebut{The performance comparison between the large loss sample selection, small loss sample selection, and random selection (ours).} }\label{tab:random_sample}
\resizebox{0.65\columnwidth}{!}{
\rebut{
\begin{tabular}{l|c|ccccc}
\thickhline
                                        & Category & CE & CE-DRW & LDAM-DRW & BS & RIDE \\ \midrule
\multirow{4}{*}{Larger Loss}            & Many                 & 67.0                     & 61.6                       & 63.1                         & 59.9                   & 67.9                     \\
                                        & Med                  & 37.1                   & 45.2                       & 45.7                         & 42.4                   & 51.2                     \\
                                        & Few                  & 7.3                    & 20.3                       & 20.3                         & 23.3                   & 25.8                     \\
                                        & All                  & 38.6                   & 43.5                       & 44.2                         & 42.8                   & 49.4                     \\ \midrule
\multirow{4}{*}{Smaller Loss}             & Many                 & 53.0                     & 53.4                       & 54.5                         & 51.2                   & 59.3                     \\
                                        & Med                  & 24.7                   & 33.0                         & 33.9                         & 36.1                   & 38.4                     \\
                                        & Few                  & 24.2                   & 32.9                       & 33.7                         & 35.4                   & 38.2                     \\
                                        & All                  & 41.6                   & 44 .0                        & 45.5                         & 45.7                   & 49.8                     \\ \midrule
\multirow{4}{*}{Random (Ours)} & Many                 & 71.6                   & 64.3                       & 67.3                         & 63.3                   & 69.2                     \\
                                        & Med                  & 42.3                   & 49.2                       & 50.4                         & 48.4                   & 52.8                     \\
                                        & Few                  & 9.4                    & 26.7                       & 21.4                         & 28.7                   & 27.3                     \\
                                        & All                  & 42.7                   & 47.7                       & 47.6                         & 47.7                   & 50.7          \\
\thickhline
\end{tabular}}}
\end{table}

==> [SM,JW] CUDA_ Curriculum of Data Augmentation for Class Imbalanced Dataset/tab/rebuttal/sensitiviy_in.tex <==
\begin{table}[ht]
\centering
\caption{\rebut{Sensitivity analysis of $\gamma$ with BS on ImageNet-LT dataset}}\label{tab:sensitivity_in}
\resizebox{0.5\columnwidth}{!}{
\rebut{
\begin{tabular}{l|cccc}
\thickhline
$\gamma$  & $0.3$   & $0.4$   & $0.5$   & $0.6$   \\ \midrule
Acc. (\%) & 51.42 & 51.59 & 51.38 & 51.24 \\
\thickhline
\end{tabular}}}
\end{table}

==> tab/rebuttal/classifier_norm.tex <==
\begin{table}[ht]
\centering
\caption{\rebut{The comparison of variance of L1 norm for class-wise linear classifier between various augmentation strategy (vanilla, AutoAugment\,\cite{cubuk2019autoaugment}, and \alg).}}\label{tab:classifier_norm}
\resizebox{1.0\columnwidth}{!}{
\rebut{
\begin{tabular}{l|ccccccccccc}
\thickhline
Augment / Epoch & 0 & 20 & 40 & 60 & 80 & 100 & 120 & 140 & 160 & 180 & 200 \\ \midrule
Vanilla (w/o Augment)         & 0.826                 & 3.018                  & 3.448                  & 3.470                   & 3.342                  & 3.202                   & 3.093                   & 3.104                   & 3.044                   & 2.967                   & 2.967                   \\
AutoAugment         & 0.819                 & 2.700                    & 3.149                  & 3.065                  & 2.958                  & 2.908                   & 2.810                    & 2.723                   & 2.646                   & 2.527                   & 2.526                   \\
\alg            & 0.821                 & 2.651                  & 2.892                  & 2.708                  & 2.502                  & 2.444                   & 2.393                   & 2.364                   & 2.297                   & 2.182                   & 2.182         \\
\thickhline
\end{tabular}}}
\end{table}
